Design of Robust and Efficient Edge Server Placement and Server Scheduling Policies: Extended Version

We study how to design edge server placement and server scheduling policies under workload uncertainty for 5G networks. We introduce a new metric called resource pooling factor to handle unexpected workload bursts. Maximizing this metric offers a strong enhancement on top of robust optimization against workload uncertainty. Using both real traces and synthetic traces, we show that the proposed server placement and server scheduling policies not only demonstrate better robustness against workload uncertainty than existing approaches, but also significantly reduce the cost of service providers. Specifically, in order to achieve close-to-zero workload rejection rate, the proposed server placement policy reduces the number of required edge servers by about 25% compared with the state-of-the-art approach; the proposed server scheduling policy reduces the energy consumption of edge servers by about 13% without causing much impact on the service quality.

==> IWQoS2021(Extended)/sections/0Abstract.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.


%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{abstract}
We study how to design edge server placement and server scheduling policies under workload uncertainty for 5G networks. We introduce a new metric called \emph{resource pooling factor} to handle unexpected workload bursts. Maximizing this metric offers a strong enhancement on top of robust optimization against workload uncertainty. Using both real traces and synthetic traces, we show that the proposed server placement and server scheduling policies not only demonstrate better robustness against workload uncertainty than existing approaches, but also significantly reduce the cost of service providers. Specifically, in order to achieve close-to-zero workload rejection rate, the proposed server placement policy reduces the number of required edge servers by about 25\% compared with the state-of-the-art approach; the proposed server scheduling policy reduces the energy consumption of edge servers by about 13\% without causing much impact on the service quality.

%As 5G takes off and user requests increase, Edge Computing (EC) provides a better user experience in the close proximity of mobile subscribers. However, server placement still need to further improve performance and reduce complexity because of the network complexity and the workload uncertainty. In addition, user requests are not always crowded. From an energy-saving perspective, we should think about on-off scheduling, which ensures energy saving without loss of performance.

%To handle workload uncertainty, we rethink resource pooling and propose a data driven approach including edge server placement and on-off scheduling, which reduces the number of rejected workload effectively while reducing algorithmic complexity. Compared with xxx, 

\end{abstract}

\begin{IEEEkeywords}
Edge Computing, Server Placement, Server Scheduling, Robust, Workload Uncertainty
\end{IEEEkeywords}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.


==> IWQoS2021(Extended)/sections/1Introduction.tex <==
\section{Introduction}
We study the edge server placement problem for 5G networks in this paper. By moving storage, compute, control, etc., closer to the network edge, Edge Computing (EC) could offer higher bandwidth, lower latency and better security to users, and thus has become a key enabling technology for 5G. As 5G takes off, deploying edge computing servers also becomes a priority for service providers.

The key challenge of edge server placement in 5G networks comes from workload uncertainty. 5G adopts \emph{small-cell deployment} to allow end users to communicate at high data rate using millimeter wave. But on the other hand, as the cell size reduces, the number of users served by each base station decreases and thus the aggregated workload at each base station becomes highly variable. One possible solution to handle such workload uncertainty is to over-provision edge computing resources based on the peak workload of all the base stations. However, this approach not only incurs high deployment and energy cost, but also leads to low average resource utilization. 

Most server placement literature~\cite{Wang2019Edge, Guo2019User,Zeng2018Edge,Li2018An,Chin2020Queuing,Cao2020Exploring, Kasi2020Heuristic, Ren2018A, guo2020user, Tero2020Edge, Xu2016Efficient, Jia2017Optimal,Yang2019Cloudlet} does not account for workload uncertainty explicitly. In general, these server placement proposals take a predicted edge workload vector as input, and compute server placement solutions with optimal expenditure, optimal access delay, or minimal energy consumption. However, we cannot keep updating server placement based on the real-time workload. When the real-time workload patterns deviate from the predictions, the performance guarantee offered by these proposals become questionable. Some recent works~\cite{Cui2020Robust, Cui2020Trading, Lu2020Robust, Khan2009Robust} studied how to design edge server placement policies that are robust to server failures. However, workload uncertainty is inherently different from server failures, and thus may need completely new handling mechanisms. 

Handling workload uncertainty is a challenging task. One may use stochastic optimization to handle workload uncertainty. However, this approach requires knowing the detailed distribution of the random workload beforehand, which can be extremely difficult to obtain.
Further, this approach may also suffer from the curse of dimensionality as the edge workload is actually a high-dimensional random vector containing thousands of entries. Another approach to handle uncertainty is robust optimization. This approach formulates uncertainty using a set, and could offer strong performance guarantee as long as the uncertainty is bounded by this set. However, finding an appropriate set for robust optimization can be difficult in practice. If we find a set that only covers a majority, (e.g., 99\%) of the workload patterns, then the robust optimization approach cannot offer any guarantee for the out-of-bound workload patterns. In contrast, if we find a set that covers all the potential workload patterns, this set can be extremely large because the workload uncertainty is heavy-tailed (see Table \ref{tab:statistics} in Section \ref{sec:workload_observation3}), drastically weakening the performance guarantee of robust optimization. Further, in some situations, it may not even be feasible to find such an uncertainty set.

We propose \textbf{RO-RP}, to explicitly account for workload uncertainty in the edge server placement problem. RO-RP is built on top of robust optimization, with newly developed techniques to handle out-of-bound workload patterns. The detailed techniques are described below:
\begin{enumerate}
    \item \textbf{Robust Optimization (RO): } Our trace analysis in Section \ref{sec:workload_observation2} suggests that the edge workload exhibits different patterns during workdays and holidays. Using robust optimization, we can \textbf{optimize server placement based on multiple representative workload patterns}. As a result, we can offer a strong performance guarantee as long as the future workload patterns are within the convex hull formed by these representative workload patterns.
    \item \textbf{Resource Pool Optimization (RP): } However, robust optimization alone cannot offer good guarantee when the future workload patterns are outside of the above convex hull. To overcome this challenge, we introduce a new concept called \textbf{resource pooling factor}. By maximizing this resource pooling factor, the impact of large workload bursts can be minimized.
    \item \textbf{Robust Rounding: } Both of the above two techniques involve solving integer programming problems, which can be computationally expensive. To reduce complexity, we first relax the integer requirement of server placement, and then propose a \textbf{smallest resource pool first} rounding approach to round a fractional solution to an integer solution. This rounding approach turns out to be more robust than other candidate rounding approaches.
\end{enumerate}

In addition to a robust edge server placement solution, we also propose server scheduling to reduce the energy consumption of edge computing. Note that the cumulative edge workload has strong diurnal patterns (see Section \ref{sec:workload_observation1}). Thus, turning off some servers (or changing servers to power-saving mode) during idle hours could potentially save significant amount of energy cost. However, toggling servers between on/off states may incur additional cost. We have explicitly accounted for the switching cost in our server scheduling formulation.

Finally, we evaluate our server placement policy based on both real traces from Shanghai Telecom and synthetic traces. Compared to the existing server placement policies, RO-RP significantly reduces the workload rejection rate given the same number of edge servers. To achieve close-to-zero workload rejection rate, RO-RP requires 25\% fewer edge servers when compared with the state-of-the-art approach. We also evaluate our server scheduling policy using the real trace. Compared to the strategy that turns on all the servers at all times, server scheduling could reduce energy consumption by 13\%.


%we find that the cumulative user requests have strong diurnal patterns, which motivates us to perform server on-off scheduling for EC. The objective is to reduce energy cost, without impacting on service quality. However, two challenges are also non-negligible: 1) The geographical distribution of edge workload is highly imbalanced and hard to predict. 2) The edge workload has remarkable uncertainty. Therefore, how to handle workload uncertainty becomes a primary focus of server placement in this paper.

%Other than robust optimization, our approach don't have to solve integer programming and adopt a \emph{relaxation and rounding} approach to reduce computational complexity. We use rejected workload metric(\S\ref{sec:rejected_workload}) to optimize server placement.
%To handling workload uncertainty, our approach is innovative in combination with resource pooling (see \S\ref{sec:resource_pooling},\S\ref{sec:reducec_algorithmic_complexity}). The primary objective of server placement is to reduce the workload rejection rate. However, when real-word workload is not similar to historical workload, some edge servers may easily get overloaded, causing some workload being rejected. Our large resource pooling strategy allocates user requests to adjacent resource pools to improve server utilization while maintaining ability to handle uncertainty, without increasing of latency. Meanwhile, we adopt the Sparse-area First approach to perform rounding as it offers the best performance.

%In addition to performance, cost is also a consideration for service providers(SPs). Our approach also takes care of other metrics: number of servers required and cost.

% To this end, we first propose a performance metric to characterize the size of the resource pool for a given server placement. XXXX

%Server placement focus more on the spatial pattern of edge demand. Edge workloads also exhibit strong diurnal patterns. In order to reduce energy consumption, we also propose to dynamically adjust the number of active servers in each edge cloud during real time. Here we can still use the above metric. XXXX

%Handling workload uncertainty is not a unique problem to edge server placement. Robust optimization is a widely used approach, and has been adopted to handle uncertainty for other problems, including service scheduling~\cite{Nguyen2020Two} in edge computing and replica server placement~\cite{Ho2006Managing} in CDN. In robust optimization, the uncertainty is modeled using a set, and the resulting solution could offer strong performance guarantee as long as the uncertainty is within the set. \textbf{However, the robust optimization based approach is hard to offer good performance for the server placement problem.} In general, it is very hard to find a meaningful set that could cover all the possible workload patterns. Even if we use the historical peak workload to construct a set, it is still possible that a future workload is even higher. Admittedly, if we consider a set that is extremely large, the likelihood of seeing an out-of-bound workload pattern is very low. In this case, the performance guarantee offered by robust optimization also becomes weak, and thus may not be useful in practice.

%We instead develop a completely new approach to handle workload uncertainty for the edge server placement problem. We introduce a new concept, called \textbf{resource pool factor} (see Section \ref{sec:resource_pooling}). 


%There are a number of factors that may affect EC server placement. First, since edge clouds are deployed in city areas, the unit cost of energy can be much higher than that of the central cloud. Second, unlike central cloud, each edge cloud is designed to serve latency-sensitive demand in close proximity, and thus may see much higher demand uncertainty in both spatial and time domains. How to handle such demand uncertainty with acceptable cost is one of the primary concern for edge server placement and scheduling. 

%Many existing works~\cite{Wang2019Edge, Guo2019User,Zeng2018Edge,Li2018An,Chin2020Queuing,Cao2020Exploring, Kasi2020Heuristic, Ren2018A, guo2020user} on EC server placement assume that each base station is only associated to the nearest edge cloud. This simplifies problem formulation, but on the other hand may increase the solution's sensitivity to demand uncertainty (see \S\ref{}). Specifically, when the EC workload of a certain base station suddenly increases, if the nearest edge cloud does not have enough additional capacity, some EC workload may be delayed or even denied, thus violating the promised Service Level Agreements (SLA).

%To provide better guarantee for SLA against demand uncertainty, the idea of resource pooling has been implicitly used in many service placement works~\cite{farhadi2019service,2018price-based,2019market-based}. Edge servers in close proximity can form a large resource pool. When some edge clouds are heavily loaded, users can benefit from offloading their requests to non-nearest edge clouds. However, how to design server placement policies that could enable better resource pooling has not yet received much attention.

% Apparently, different server placement strategies may have significant impact on resource pooling. Consider the simple example in Fig. \ref{fig:motivation}. The predicted EC workloads at the base stations $A$ and $B$ are both $10$, while the real time workloads turn out to be $8$ and $12$. If we deploy $10$ units of computing resources at $A$ and $B$ each (see Fig. \ref{fig:motivation:a}), then in real time, $2$ units of $B$'s workload cannot get served in a timely fashion owing to the fact that 1) $B$'s MEC servers are already fully utilized, and thus cannot serve $B$'s burst; 2) $A$ is too far from $B$, and thus cannot serve $B$'s burst either. On the other hand, if we deploy computing resources at the base stations $C$ and $D$ (see Fig. \ref{fig:motivation:b}), the computing resources of $C$ and $D$ can form a larger resource pool to serve the workloads from both $A$ and $B$, because $C$ and $D$ are both within the acceptable distance from $A$ and $B$. Then, as $B$'s workload bursts from $10$ to $12$, we can offload $2$ units of workload from the edge cloud $D$ to the edge cloud $C$. As a result, the SLA for the users at the base station $B$ may not be impaired any more. 



%As a byproduct of this work, we also map the integer programming problem to a min-cost-flow problem, which can be solved efficiently in polynomial time.

==> IWQoS2021(Extended)/sections/2Background.tex <==
\section{Related Work}\label{sec:related_work}
Prior work has studied how to deploy edge servers based on workload distribution. However, the workload distribution may not be accurate. Workload uncertainty may have a big impact on the eventual network performance, but unfortunately has not yet received much attention in the existing literature.

Many server placement proposals~\cite{Wang2019Edge, Guo2019User,Zeng2018Edge,Li2018An,Chin2020Queuing,Cao2020Exploring, Kasi2020Heuristic, Ren2018A, guo2020user} have assumed that each base station can be only associated with one edge cloud in their formulations. With this assumption, many standard algorithms, e.g., k-means clustering algorithm, set cover algorithm, etc., can be used to design heuristic solutions for the server placement problem. However, this formulation is inherently non-robust to demand uncertainty. Whenever the workload of a base station bursts, the edge cloud that serves this base station has to bear the burden by itself. In fact, for a given server placement, EC users do benefit from offloading their job requests to multiple edge clouds\cite{farhadi2019service, urgaonkar2015dynamic}. There does exist literature~\cite{Tero2020Edge, Xu2016Efficient, Jia2017Optimal,Yang2019Cloudlet} that allows serving workload from the same base station in different edge clouds. However, workload uncertainty is not considered therein.

To improve the robustness of edge server placement, \cite{Cui2020Robust, Cui2020Trading, Lu2020Robust, Khan2009Robust} studied how to account for server failures in their server placement formulations. However, workload uncertainty is inherently different from server failures, and may happen much more frequently in real time.

One natural idea to deal with workload uncertainty is to use robust optimization. This idea has been used to study the service scheduling problem~\cite{Nguyen2020Two} in EC and the replica server placement problem~\cite{Ho2006Managing} in CDN. However, robust optimization cannot offer any guarantee when the workload is outside of the predicted set. Note that, unlike service scheduling, server placement results cannot be adjusted based on the real-time workload.

%when we directly apply robust optimization to the server placement problem, the results do not seem promising (see \S\ref{}).

In addition to the server installation cost, energy also accounts for a big portion of the cost for edge computing. The energy-optimization literature on edge computing mostly focuses on the edge/IoT devices~\cite{liu2016delay, mao2017survey, lim2018camthings}, but not on the edge servers. In this paper, we study how to perform server on-off scheduling for edge computing to save energy cost. As far as we know, this server scheduling problem was only studied in data centers~\cite{Lin2011Dynamic,goiri2010energy,duy2011prediction,dayarathna2015data}, but has never been explored in edge computing. The biggest difference is that we need to account for the collaboration among different edge clouds when we study server scheduling in edge computing.

\begin{comment}
\cpr{
To serve data-intensive applications (e.g., augmented reality, video analytic) from  the  edge, \cite{farhadi2019service} proposed a two-time-scale solution for joint service placement and request scheduling, developed a polynomial-time service placement algorithm.
}

\cite{urgaonkar2015dynamic}
\cite{Tero2020Edge}.

\cpr{Cloudlets~\cite{Satyanarayanan2013The,satyanarayanan2009case,satyanarayanan2014cloudlets,verbelen2012cloudlets} reduces end-to-end latency of cloud offload from mobile devices for applications that are resource-intensive and latency-sensitive, giving mobile users the illusion that they’re directly interacting with the cloud.}

\cpr{
\cite{Nguyen2020Two} proposed a two-stage adaptive robust optimization framework, which depends on column-and-constraint generation method, a master problem and a max-min problem. \cite{Nguyen2020Two} contains a complex MILP problem so that the solution time needs to be tolerated.
}

\cpr{Edge cloud can be deployed in two architecture~\cite{WANG2020308}. One is flat deployment, which only deploy edge clouds along with the base stations. The other is hierarchical deployment, which deploy an edge cloud at the regional central office.}

\cite{Tero2020Edge} optimizes server placement by minimizing the total distance between edge servers and workload. However, the formulation in \cite{Tero2020Edge} is non-convex, and the proposed solution therein offers no optimally guarantee. 

\cite{Wang2019Edge} uses mix integer programming to optimize server-workload distance and access delay. However, the computational complexity of mix integer programming can be prohibitively high as the problem size increases.

\cite{Zeng2018Edge, Guo2019User, Li2018An, Chin2020Queuing, Kasi2020Heuristic, Ren2018A} formulates the edge server placement problem with latency constraints using mix integer programming, but only provides heuristic algorithms, i.e., K-means, greedy, simulated annealing, genetic algorithms, etc., to solve the formulation with tolerable algorithmic complexity.

\cite{Jia2017Optimal} does not consider demand uncertainty.


\cite{Cui2020Robust, Cui2020Trading} studies the robust placement problem by maximizing the possibility of take-over under server failures. Mix integer programming and an approximation algorithm are proposed. However, the approximation ratio grows linearly with respect to the number of servers.

\cite{Cao2020Exploring} jointly optimizes server placement and task scheduling using integer linear programming in the offline stage, and fine tunes the task scheduling based on the real arrival rate in the online stage.

\cite{Lu2020Robust} maximizes the workload that can be processed when at most $k$ servers fail. They prove that their objective function is monotone submodular, which is used to develop a polynomial complexity algorithm with provable constant approximation ratio.


Cloudlet placement \cite{Xu2016Efficient} is similar to server placement in edge computing. Still, heuristic algorithms are used.

Energy consumption is critical \cite{Li2018An, Yang2019Cloudlet}

\cite{Yang2019Cloudlet} formulates MILP problem, and then solves with bender's decomposition

\cite{Nguyen2020Two} uses two-stage robust optimization to place services under uncertainty.

need a table 

1 minimize cost

2 Improve robustness

3 

Robust optimization for 

Robust CDN replica placement techniques
\cite{Ho2006Managing} handles uncertainty

\cite{Khan2009Robust} handles failure


\subsection{The drawback of following scheduling}
review some papers

\subsection{The drawback of day-night scheduling}
review some papers

\subsection{The motivation and advantage of our approach}
generalize

Inspired by the analysis of the telecom dataset.

The importance of resource pooling.

The limitation of previous researches' resource pools.

Resource pooling for server placement.

Resource pooling for server on-off scheduling.

\end{comment}



==> IWQoS2021(Extended)/sections/3WorkloadAnalysis.tex <==
\section{Workload Analysis}\label{sec:workload_analysis}


\begin{table*}[!htb]
\centering
\caption{The statistics of workload and inter-arrival time over a time span of six months.}
\label{tab:statistics}
\begin{tabular}{llllllllllllll}
\hline
                   & Max      & Average & std   & 99.999\% & 99.99\%  & 99.9\%  & 99\%   & 90\%   & 80\%  & 70\%  & 60\%  & 50\%  & 40\% \\ \hline
Workload           & 40877    & 2314 & 3283  & 27144   & 10804   & 10800  & 10796 & 8857  & 3910 & 2097 & 1216 & 728  & 499 \\
Inter-arrival time & 13953857 & 7174 & 64180 & 7246866 & 2584387 & 584956 & 82414 & 10731 & 5001 & 3002 & 1990 & 1374 & 899 \\ \hline
\end{tabular}
\end{table*}



%Although the existing literature has proposed several server placement strategies for edge computing, there lacks a comprehensive trace study that helps 

The appropriate design of server placement policies requires a deep understanding of the potential workload patterns of EC. However, EC has not seen widespread deployment yet, and thus there may not be any real data for its workloads. Instead, we perform workload analysis based on Shanghai Telecom dataset~\cite{Wang2019Edge,wang2019qos,guo2020user,wang2019delay}, which includes communication records collected about 3042 base stations and 6236620 user requests. We believe that the workload patterns of these communication records can provide a good estimate for the workload patterns of EC.

%3233 base stations and 6952921 user requests, where there are valid 

%\cpr{TODO: modify the next sentence.}. Admittedly, these communication records are not really edge computing workloads. Nevertheless, we expect that the workload patterns of these communication records might be similar to the workload patterns of edge computing.

\subsection{Observation 1: The cumulative workload has strong diurnal patterns}\label{sec:workload_observation1}
We study how the cumulative workload across all base stations in Shanghai varies at different times of a day using a consecutive of 30 days of data. As shown in Fig.~\ref{fig:traffic_demands}, the total number of requests are the lowest from midnight to about 6:00am every day. As people get up around 6:00-8:00am, the requests rise and peak at around 6:30-7:30am. Then, the requests are relatively consistent until 20:00pm, after which the requests gradually decrease. Another observation from the curves is that the number of requests on workdays (solid lines) is generally higher than that on holidays (dashed lines). This implies that one should not use workday's workload patterns to predict the workload patterns on holidays, and vice versa.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{images/traffic_analysis_table.pdf}
%     \caption{Number of Requests at different time of the day during one month.}
%     \label{fig:traffic_demands}
% \end{figure}

\begin{figure*}[!htb]
    \centering
    \subfigure[Number of Requests at different time of the day during one month.] {
        \label{fig:traffic_demands}
        \includegraphics[width=0.64\columnwidth]{images/traffic_analysis_table.pdf}
    }
    \subfigure[Hour-level workload variation for two consecutive weeks.] {
        \label{fig:traffic_delta:a}
        \includegraphics[width=0.64\columnwidth]{images/traffic_delta_analysis.pdf}
    }
    \subfigure[Hourly workload statistics for each base station over a period of 6 months.] {
        \label{fig:traffic_delta:b}
        \includegraphics[width=0.64\columnwidth]{images/step3_draw_station_mean_std.png}
    }
\caption{Data set analysis.}
\label{fig:traffic_delta}
\end{figure*}

% \begin{figure*}[!h]
%     \centering
%     \subfigure[00:00-08:00] {
%         \label{fig:one_day_demands_map:a}
%         \includegraphics[width=0.63\columnwidth]{images/hour0.png}
%     }
%     \subfigure[08:00-15:59] {
%         \label{fig:one_day_demands_map:b}
%         \includegraphics[width=0.63\columnwidth]{images/hour8.png}
%     }
%     \subfigure[16:00-23:59] {
%         \label{fig:one_day_demands_map:c}
%         \includegraphics[width=0.63\columnwidth]{images/hour16.png}
%     }
%     \caption{Requests distribution at different times of the day.}
%     \label{fig:one_day_demands_map}
% \end{figure*}

\begin{figure}[!h]
    \centering
    \subfigure[12:00-14:00 on Holiday] {
        \label{fig:workday_weekend0}
        \includegraphics[width=0.8\columnwidth]{images/workday_weekend_0.png}
    }
    \subfigure[12:00-14:00 on Workday] {
        \label{fig:workday_weekend3}
        \includegraphics[width=0.8\columnwidth]{images/workday_weekend_1.png}
    }
    \caption{Requests distribution at different days.}
    \label{fig:requests_distribution}
\end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/requests_duration.pdf}
%     \caption{Duration distribution of each base station requests.}
%     \label{fig:requests_duration}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/requests_inter_arrival.pdf}
%     \caption{Inter-arrival time distribution of each base station requests.}
%     \label{fig:requests_inter_arrival}
% \end{figure}


The strong diurnal patterns of edge workload motivates us to \textbf{perform server on-off scheduling} for EC. The objective is to reduce energy cost, without impacting on service quality.

\subsection{Observation 2: The spatial workload patterns of different days can be highly skewed and dramatically different}\label{sec:workload_observation2}
As shown in Fig.~\ref{fig:requests_distribution}, we randomly pick a holiday and a workday, and study their workload patterns at the same time of a day. Fig.~\ref{fig:traffic_demands} demonstrates that the total workloads at workdays and holidays are approximately the same for most times of a day. However, when we compare the spatial workload distributions in Fig.~\ref{fig:requests_distribution}, the workload patterns are apparently different. This observation suggests that we should \textbf{use multiple different workload patterns to compute server placement solutions}.

Another observation from Fig.~\ref{fig:requests_distribution} is that the workload patterns are highly skewed, with much higher workload in the central area of Shanghai. Hence, traffic agnostic server placement strategies may not perform well, which is verified via simulation in Section \ref{sec:compare_server_placement}.

% account for such highly imbalanced geographical distribution. However, workload-aware server placement is not straight-forward, due to the following reasons:
% \begin{enumerate}
%     \item Although the cumulative workload is relatively stable, the workload at each base station can be highly variable;
%     \item Server placement result is determined at the planning stage, and is hard to change on demand.
% \end{enumerate}

\subsection{Observation 3: The edge workload is highly bursty}\label{sec:workload_observation3}

To understand the burstiness of edge workload, we analyze the workload sizes and the inter-arrival times of all the requests at each base station over a time span of six months. Table~\ref{tab:statistics} summarizes the average, standard deviation and percentile values of these two metrics. Note that the inter-arrival time is heavy tailed, meaning that it is possible for a base station to receive a large request after being idle for a long period of time.

% \cpr{del? Fig.~\ref{fig:requests_duration} shows that most of workload is less than 800, and workload from 800 to 2000 and longer than 10600 are also obvious. For the convenience of presentation, we selected three representative base stations for drawing Fig.~\ref{fig:requests_inter_arrival}. The inter-arrival time of different base stations has obvious differences, which makes it very difficult to accurately predict the workload. }

% \begin{figure}[!htb]
%     \centering
%     \subfigure[Hour-level workload variation for two consecutive weeks.] {
%         \label{fig:traffic_delta:a}
%         \includegraphics[width=0.8\columnwidth]{images/traffic_delta_analysis.pdf}
%     }
%     \subfigure[Hourly workload statistics for each base station over a period of 6 months.] {
%         \label{fig:traffic_delta:b}
%         \includegraphics[width=0.8\columnwidth]{images/step3_draw_station_mean_std.png}
%     }
% \caption{}
% \label{fig:traffic_delta}
% \end{figure}

Since edge workload is highly bursty, accurately predicting edge workload can be very difficult. For example, we can use historical workday/holiday patterns to predict future workload. For the $t$-th hour in every day, we could compute the following workload variation ratio:
$$V_t = \frac{\sum_{m=1}^M{|w_m(t)-w_m^{'}(t)|}}{\sum_{m=1}^M{w_m^{'}(t)}},$$
where $w_m(t)$ is the total workload of the $m$-th base station in the $t$-th hour of the day, and $w_m^{'}(t)$ is the total workload of the $m$-th base station in the $t$-th hour seven days ago. From Fig.~\ref{fig:traffic_delta:a}, we see that the workload variation ratio can be as large as $70\%$. Hence, using historical patterns to predict future workload can be highly inaccurate.

%, even though we evaluate different times of the day according to our routine.

We are also interested in the relationship between the average workload and the workload uncertainty. For every base station and every hour in a week, we collect a sequence of workload values over 6 months with one value per week. We then compute the average value and the standard deviation for every workload sequence, and plot them in Fig.~\ref{fig:traffic_delta:b}. From this figure, we can see that the workload's worst-case standard deviation grows approximately linearly with respect to its average value. However, the range of the standard deviation values is pretty large, and thus there may not be a rule of thumb to accurately predict the workload uncertainty.

%have some aggregation effect, but there is no general law, and it is difficult to predict.

The above analysis demonstrates that edge workload is highly variable. Thus, \textbf{how to handle workload uncertainty} becomes a primary focus in this paper. 


%Apparently, The number of requests for services decreases at midnight (from 0:00am to 8:00am), which in line with the regularity of people’s work and rest. 

%Further, we count the request demands for each hour of every day in a month and the cumulative effect presents a more detailed pattern, shown in Fig.~\ref{fig:traffic_demands:a}. From midnight to 5:00am, most people are sleeping with the fewest requests. From the time when people get up at 6 o'clock, requests suddenly increase, and peak at 7 o'clock. Fig.~\ref{fig:traffic_demands:b} shows that the daily request demands are relatively consistent, and the overall demands of workdays is greater than that on weekends. This inspired us to only use the demands of this day last week to make predictions, instead of using too complex algorithms to reduce complexity.

%\subsection{Observation 2: Edge workload is hard to predict}
%However, from Fig.~\ref{fig:traffic_demands:b}, we can find that there are daily peaks and troughs of request demands, but the overall trend is variation on some days. In order to explore the details of the amount of variation, we calculated the amount of workload variation in the corresponding hour period for each two consecutive weeks, shown in Fig.~\ref{fig:traffic_delta:a}. Specifically, workload variation ratio $$V_t = \frac{\sum_{s=1}^n{|d_s(t)'-d_s(t)|}}{\sum_{s=1}^n{d_s(t)}}$$, where $V_t$ denotes the amount of workload variation corresponding to a certain hour in the two consecutive weeks, $d_s(t)$ denotes the workload duration of base station $s$ on the $i$-th hour on the day of this week, and $d_s(t)'$ denotes of the consecutive next week.

%In addition, we calculated the hourly workload statistics for each base station over a period of 6 months shown in Fig.~\ref{fig:traffic_delta:b}. Where the mean and standard deviation have a similar linear correlation, therefore the objective of (\ref{formulation:server_placement_robustification}) can adapt to the law.



% \subsection{Observation 3: New base station are being deployed.}
% The number of base stations from June 1 to June 10 was 2678, with an increase of 206 from June 11 to June 20 and 158 from June 21 to June 30. No new base stations were added from July to December.

% New base station does not have any historical traffic data. How can we estimate its potential demand?


==> IWQoS2021(Extended)/sections/4SystemModel.tex <==
\section{Model}
We study edge server placement from a service provider's aspect. A service provider (SP) is responsible for managing the base stations, the central cloud and the edge servers (see Fig. \ref{fig:architecture:a}), with an objective to provide ubiquitous communication and computation services to its users. Users access SP's network through base stations, usually via wireless links. The base stations and the central cloud are typically interconnected through wired links. As we go into the 5G era, when millions of devices connect to the network, and data from each device floods in, edge computing also becomes critical to provide low latency, high reliability, and immense bandwidth.

In general, edge computing consists of two stages: server placement and service scheduling. For server placement, the SP needs to determine where to deploy servers and how many servers to deploy. Typically, edge servers are co-located with base stations. Server placement usually happens at the planning stage. For service scheduling, the SP is responsible for routing users' edge computing requests to nearby edge servers in real time. In this paper, we focus on server placement. Note that running edge servers may incur high energy cost. To reduce energy consumption, we introduce an additional stage, i.e., server on-off scheduling, to make an on-off schedule for edge servers based on predicted workloads. The overall workflow of edge computing is depicted in Fig. \ref{fig:architecture:b}.

\begin{figure}[!htbp]
    \centering
    \subfigure[Edge computing network.] {
        \label{fig:architecture:a}
        \includegraphics[width=0.46\columnwidth]{images/station_drawio.pdf}
    }
    \subfigure[Overall workflow.] {
        \label{fig:architecture:b}
        \includegraphics[width=0.46\columnwidth]{images/stage_structure.pdf}
    }
\caption{Overall Architecture.}
\label{fig:architecture}
\end{figure}

\subsection{Mathematical Models}
Let $\{B_1, B_2,...,B_M\}$ denote the set of base stations (BSs) in an 5G network, where $M$ is the total number of base stations. Assume time is slotted. $w_{m}(t)$ denotes the total edge computing workload of BS $B_m$ at slot $t$. The workloads at different base stations form a workload vector $w(t)=[w_{m}(t),m=1,2,...,M]$. Since the edge workload $w_{m}(t)$ has stringent latency requirements, such workload can be only processed by the edge servers deployed at the BS $B_m$ or the nearby BSs of $B_m$. In this paper, we use $\Omega_m$ to denote the set of BSs whose edge servers can serve the workload of the BS $B_m$.
%$$\Omega_{m}=\{i=1,...,M:\text{The communication latency %between }B_i\text{ and }B_m\text{ is less than }\delta\}$$
%\zx{$\Omega_{m}(\delta)=\{i=1,...,M:\text{The latency between }B_i\text{ and }B_m\text{ is less than }\delta\}???$}

\noindent\textbf{Remark on $\Omega_m$:} One can define $\Omega_m$ using different approaches, including latency requirement, hop-count requirement, distance requirement, $k$-nearest neighbor requirement, etc. The methodology in this paper works for all the possible definitions of $\Omega_m$.

\subsubsection{Server Placement}
Server placement typically happens at the planning stage. Once the edge servers are deployed, it may not be easy to change the server deployment. Hence, server placement must be robust against the potential workload variations. The easiest approach to deal with workload variations is to over-provision edge servers. However, this approach increases both equipment cost and energy cost. In this paper, given a historical trace of workload vectors, we study how to assign a total number of $K$ servers to each BS, such that
\begin{equation}\label{eqn:total_servers}
    S_{1} + S_{2} + \cdots + S_{M} = K,\text{ where $S_m$'s are integers},
\end{equation}
where $S_m$ is the number of edge servers to be deployed at the BS $B_m$.

%SPs typically use a historical-average or a historical-max workload vector, denoted by $[w_{m},m=1,2,...,M]$, to compute a server placement solution.

\subsubsection{Service Scheduling}
Service scheduling happens at the real time stage. At time $t$, for the workload $w_m(t)$ at the BS $B_m$, the objective of service scheduling is to determine the fraction $u_{mn}(t)$ of the workload $w_m(t)$ that is assigned to the base station $B_n\in\Omega_m$. Clearly,
\begin{equation}\label{eqn:demand_split}
\left\{ 
\begin{array}{lc}
\sum_{B_n\in\Omega_m}u_{mn}(t)=1,\text{ for }m=1,2,...,M,\\
0\leq u_{mn}(t)\leq 1\text{ and } u_{mn}(t)=0,\text{ for }B_n\notin \Omega_{m}.
\end{array}
\right. 
\end{equation}

\subsubsection{Server On-off Scheduling}
Server on-off scheduling happens in-between server placement and service scheduling. Fig.~\ref{fig:traffic_demands} suggests that the cumulative edge workload has daily peaks and troughs. Server placement needs to account for the daily peaks. However, keeping all the servers always \emph{on} incurs significant energy cost, especially during idle hours. Let $S(t)=[S_m(t),m=1,2,...,M]$, where $S_m(t)$ is the number of active servers at the BS $B_m$ at time $t$. The objective of server on-off scheduling is to reduce energy cost, without impacting on users' service quality. Clearly,
\begin{equation}\label{eqn:active_servers}
S_m(t)\leq S_m,\forall{m=1,2,...,M}\text{ and }t.
\end{equation}

\subsection{Performance Metrics}
While we design server placement and server on-off scheduling strategies, we are interested in optimizing the following three performance metrics.

\subsubsection{Rejected Workload}
\label{sec:rejected_workload}
When edge servers run out of resources to serve some portion of edge workload, such edge workload is considered as rejected. (Offloading this workload to the central cloud may violate latency requirement.) This could happen when the real-time workload $w(t)=[w_1(t),w_2(t),...,w_M(t)]$ bursts at some BSs. Given the numbers of active servers $S(t)$ and the workload vector $w(t)$, the total amount of rejected workload can be computed by
\begin{equation}\label{formulation:rejected_workload}
\boxed{
\begin{aligned}
\min_{u_{mn}(t)} & \hspace{3mm}\sum_{n=1}^M\max\left\{0,\sum_{m=1}^M w_m(t)u_{mn}(t)-C S_n(t) \right\} &\\
\text{s.t.}& \hspace{3mm} u_{mn}(t)\text{ satisfy (\ref{eqn:demand_split}),}&
\end{aligned}
}
\end{equation}
where $C$ is the capacity of one server. Note that $\max\left\{0,\sum_{m=1}^M w_m(t)u_{mn}(t)-CS_n(t) \right\}$ is the total rejected workload at the BS $B_n$. Solving (\ref{formulation:rejected_workload}) gives the minimum possible amount of workload to be rejected.

\subsubsection{Number of Servers Required}
From service providers' aspect, rejecting EC requests is highly undesirable, because they may lose customer loyalty. Then, another important metrics arises, i.e., what is the minimum number of servers required in order to guarantee zero workload rejection rate? Certainly, this number depends on the server placement strategy and the workload patterns. In Section \ref{sec:compare_server_placement}, we will use extensive simulation to obtain an estimate of this metric for different server placement strategies.

\subsubsection{Cost}
The cost of edge servers consists of two parts:
\begin{itemize}
    \item Server running cost $E_r+E_w\cdot x$, where $E_r$ is the energy cost of running an idle server for one time slot, and $E_w$ is the energy cost per workload unit. Note that $E_r$ may account for more than $50\%$ of the energy cost in a server~\cite{powerconsumption}. 
    \item Switching cost $E_s$, which models the cost of toggling a server between on/off states. As stated in~\cite{Lin2011Dynamic}, if only energy cost matters, then $E_s$ is on the order of the cost of running a server for a few seconds to several minutes; if the increased wear-and-tear is accounted for, then $E_s$ becomes on the order of the cost of running a server for a hour. In this paper, we use the latter to measure the switching cost $E_s$.
\end{itemize}

Note that the total energy cost of all the workload equals $E_w\sum_{m=1}^M\sum_t w_m(t)$, which is out of our control. Hence, in this paper, we mainly focus on the idle-server cost and the switching cost, which in total can be calculated as
\begin{equation}\label{eqn:cost}
    W=\sum_{m=1}^M\sum_t\bigg(E_r\times S_m(t) + E_s\times(S_m(t)-S_m(t-1))^+\bigg),
\end{equation}
where $x^+=\max\{0,x\}$. Clearly, if we choose not to perform server on-off scheduling, then the switching cost becomes zero, but the running cost increases.




==> IWQoS2021(Extended)/sections/5ServerScheduling.tex <==
\section{Server Placement}\label{sec:server_placement}
%Base stations, edge servers, cloud data centers and mobile devices together constitute today's Internet of Everything. Their network constitutes a graph structure $G=(V, E)$ shown in Fig.~\ref{fig:base_station}. Where $V=B\cup S$, $B$ is the set of base stations and $S$ is the set of edge servers. A base station may not deploy servers, or deploy many servers, which is determined by our server placement approach. $E$ represents the set of links between a base station and another base station or cloud data centers. When different numbers of IoT devices move to different locations to send requests, the workload of base stations in different locations will be different. 

The primary objective of server placement is to reduce the workload rejection rate. Since this metric is closely related to service scheduling, our server placement strategy will account for the effect of service scheduling. 

\subsection{A robust joint optimization approach}\label{sec:robust_optimization}
Owing to the fact that edge workload exhibits different patterns at different time of different days, our first idea is to use robust optimization to compute a server placement solution. Specifically, given a sequence of historical workload vectors, we pick multiple representative workload vectors using the following steps:
\begin{description}
\item[Step 1] Divide historical workload vectors into $L$ groups such that the workload vectors in the same group are all 1) from workdays or holidays, and 2) from the same time period (e.g., 8:00-11:59am) of a day.
\item[Step 2] Compute an average workload vector $w^l=[w_m^l,m=1,2,...,M]$ for the $l$-th group of workload vectors\footnote{We have also tried using the component-wise max workload vector to compute a server placement solution. However, our simulation results in Section \ref{sec:average-max-comparison} cannot give any conclusive answer that one option is better than another. Hence, one may use a different approach to compute representative workload vectors.}. Note that the following analysis also works for other choices of workload vectors.
\end{description}
In total, we obtain $L$ workload vectors.

For each workload vector $w^l$, we introduce service scheduling variables $u^l=[u_{mn}^l, m,n=1,2,...,M]$ satisfying (\ref{eqn:demand_split}). Then, we jointly optimize the server placement variables $S=[S_m,m=1,2,...,M]$ satisfying (\ref{eqn:total_servers}) and the service scheduling variables $[u^1,u^2,...,u^L]$. 

For each workload vector $w^l$ and the corresponding service scheduling variables $u^l$, it is easy to obtain the total workload allocated to the BS $B_n$, i.e., $\sum_{m=1}^M w_m^l u_{mn}^l$. To reduce the likelihood of workload rejection, we impose the following constraint that restricts the edge server utilization to be less than $\beta$ for any BS $B_n$ and any workload vector $w^l$:
\begin{equation}\label{eqn:server_capacity}
\sum_{m=1}^M w_m^l u_{mn}^l\leq S_n C \beta,\text{ for any }B_n\text{ and }w^l.
% \left\{ 
% \begin{array}{c}
% u_{11}w_1+u_{21}w_2+\cdots+u_{M1}w_M \leq S_{1}*C*\beta, \\ 
% u_{12}w_1+u_{22}w_2+\cdots+u_{M2}w_M \leq S_{2}*C*\beta,  \\ 
% \cdots\cdots\cdots\cdots  \\
% u_{1M}w_1+u_{2M}w_2+\cdots+u_{MM}w_M \leq S_{M}*C*\beta.  \\ 
% \end{array}
% \right. 
\end{equation}
Then, the overall formulation is given as
\begin{equation}\label{formulation:server_placement}
\boxed{
\begin{aligned}
\min_{S,u^l,\beta} & \hspace{20mm}\beta &\\
\text{s.t.}& \hspace{3mm} S\text{ satisfy (\ref{eqn:total_servers}),}&\\
& \hspace{3mm} S,u^l,\beta\text{ satisfy (\ref{eqn:demand_split})(\ref{eqn:server_capacity}) for }l=1,2,...,L.&
\end{aligned}
}
\end{equation}

\noindent\textbf{Understanding the performance guarantee of (\ref{formulation:server_placement}):} Let $\hat{S},\hat{u}^l,\beta^*$ be the optimal solution of (\ref{formulation:server_placement}). Consider a future workload vector $w\leq\sum_{l=1}^L\lambda_l w^l$, where $\lambda_l\geq 0, l=1,2,...,L$ and $\sum_{l=1}^L \lambda_l=1$. In other words, the workload vector $w$ is bounded by the convex hull of the workload vectors $[w^1,w^2,...,w^L]$. We construct the service scheduling variable $u$ for $w$ as follows:
\begin{equation}\label{eqn:calculateu}
u_{mn}=\sum_{l=1}^L\frac{\lambda_l w_m^l}{\sum_{i=1}^L \lambda_i w_m^i}\hat{u}_{mn}^l
\end{equation}
It is easy to check that $u$ satisfies (\ref{eqn:demand_split}). Further,
\begin{eqnarray}
\sum_{m=1}^M w_m u_{mn}&=&\sum_{m=1}^M w_m \sum_{l=1}^L\frac{\lambda_l w_m^l}{\sum_{i=1}^L \lambda_i w_m^i}\hat{u}_{mn}^l\nonumber\\
&\leq&\sum_{m=1}^M\sum_{l=1}^L\lambda_l w_m^l\hat{u}_{mn}^l=\sum_{l=1}^L\lambda_l\sum_{m=1}^M w_m^l\hat{u}_{mn}^l\nonumber\\
&\leq&\sum_{l=1}^L\lambda_l \hat{S}_n C\beta^*=\hat{S}_n C\beta^*.\nonumber
\end{eqnarray}
Hence, the workload $w$ is supportable by the server placement solution $\hat{S}$ with max server utilization no greater than $\beta^*$.

\noindent\textbf{Understanding the drawback of (\ref{formulation:server_placement}):} 
When future workload vectors are bounded by the convex hull of $[w^1,w^2,...,w^L]$, the above analysis indicates that (\ref{formulation:server_placement}) can offer strong performance guarantee. However, some future workload vectors can be out of bound, owing to the fact that edge workload is highly bursty. Certainly, one can increase the convex hull by scaling up the representative workload vectors $[w^1,w^2,...,w^L]$. Unfortunately, $\beta^*$ will also increase, making the performance guarantee of robust optimization weaker. Further, if $\beta^*>1$, then the performance guarantee becomes useless.


%However, the performance of the above robust optimization based approach performs strictly worse than our resource pooling based approach (see \S\ref{}). The reason is that, although using multiple workload vectors creates a relatively large convex workload set, it is still possible that the real-time workload is outside the workload set, in which case robust optimization can no longer provide performance guarantee. 

%This formulation guarantees good performance when the real-time workload $w(t)$ is similar\footnote{``Similar'' means that $\frac{w_1(t)}{w_1}\approx \frac{w_2(t)}{w_2} \approx \cdots \approx \frac{w_M(t)}{w_M}$.} to the workload vector $w$. However, when the real-time workload vector $w(t)$ deviates significantly from $w$, some edge servers may easily get overloaded, causing some workload being rejected.

%\noindent\textbf{Remark:} 

%Our server placement formulation (\ref{formulation:server_placement}) is slightly different from the formulations in literature~\cite{Wang2019Edge, Guo2019User,Zeng2018Edge,Li2018An,Chin2020Queuing,Cao2020Exploring, Kasi2020Heuristic, Ren2018A, guo2020user, Tero2020Edge, Xu2016Efficient, Jia2017Optimal,Yang2019Cloudlet}. Instead of formulating the server access latency as an objective function, we enforce the latency requirement as the constraint ``$u_{mn}=0\text{ for }n\notin \Omega_{m}(\delta)$''. Clearly, this subtle difference offers stronger guarantee to the server access latency. More importantly, this formulation allows us to develop a polynomial algorithm that can compute a close-to-optimal solution of (\ref{formulation:server_placement}) (see \S\ref{}). In contrast, existing literature on server placement usually rely on heuristic ideas that have a clear gap between the optimal solution.

\subsection{Handling Out-of-bound Workload with Resource Pooling}
\label{sec:resource_pooling}
\noindent\textbf{Intuition:} We first introduce the concept of \emph{resource pool}. For the workload at the BS $B_m$, its \emph{resource pool} is defined as the total amount of server resources that can serve the workload, which equals to $\sum_{B_n\in \Omega_m}S_n$. To understand how resource pooling helps mitigate the impact of out-of-bound workload, we consider the motivation example in Fig. \ref{fig:motivation}. The predicted MEC workloads at the base stations $A$ and $B$ are both $10$, while the real time workloads turn out to be $8$ and $12$. If we deploy $10$ units of computing resources at $A$ and $B$ each (see Fig. \ref{fig:motivation:a}), then in real time, $2$ units of $B$'s workload will be rejected owing to the fact that 1) $B$'s MEC servers are already fully utilized, and thus cannot serve $B$'s burst; 2) $A$ is too far from $B$, and thus cannot serve $B$'s burst either. On the other hand, if we deploy computing resources at the base stations $C$ and $D$ (see Fig. \ref{fig:motivation:b}), the computing resources of $C$ and $D$ can serve the workloads from both $A$ and $B$, because $C$ and $D$ are both within an acceptable distance from $A$ and $B$. As a result, the resource pools of both $A$ and $B$ increases from $10$ to $20$. Then, as $B$'s workload bursts from $10$ to $12$, we can offload $2$ units of workload from the edge cloud $D$ to the edge cloud $C$. With an increase resource pool, the workload from the base station $B$ will not be rejected any more. 
\begin{figure}[!htb]
    \centering
    \subfigure[Small resource pool.] {
        \label{fig:motivation:a}
        \includegraphics[width=0.46\columnwidth]{images/motivation1.pdf}
    }
    \subfigure[Large resource pool.] {
        \label{fig:motivation:b}
        \includegraphics[width=0.46\columnwidth]{images/motivation2.pdf}
    }
\caption{Motivation example of resource pooling.}
\label{fig:motivation}
\end{figure}

\noindent\textbf{Formulation:} Motivated by the above example, we introduce a resource pooling factor $\eta$, such that
\begin{equation}\label{eqn:resource_pool_factor}
    \eta \max_{l=1}^L \{w_m^l\} \leq \sum_{B_n\in \Omega_m}S_n.
\end{equation}
Then, we compute the server placement result by maximizing the resource pooling factor $\eta$:
\begin{equation}\label{formulation:server_placement_robustification}
\boxed{
\begin{aligned}
&\hspace{-5mm}\textbf{Maximize resource pooling factor:}&\\
\max_{S,u^l,\eta} & \hspace{20mm} \eta &\\
\text{s.t.}& \hspace{3mm} S,\eta \text{ satisfy (\ref{eqn:total_servers})(\ref{eqn:resource_pool_factor}),}&\\
& \hspace{3mm} S,u^l,\beta^*\text{ satisfy (\ref{eqn:demand_split})(\ref{eqn:server_capacity}) for }l=1,2,...,L.&
\end{aligned}
}
\end{equation}
Note that our server placement policy involves two steps: 1) compute $\beta^*$ using the \emph{robust optimization} formulation (\ref{formulation:server_placement}); 2) optimize \emph{resource pooling} based on (\ref{formulation:server_placement_robustification}). Hence, we will also use \textbf{RO-RP} to represent our server placement policy.

\noindent\textbf{Understanding the performance guarantee of (\ref{formulation:server_placement_robustification}):}
Let $S^*, \eta^*$ be the optimal solution of (\ref{formulation:server_placement_robustification}). 
Consider an arbitrary workload vector $w$. If the workload vector $w$ is within the convex hull of $[w^1,w^2,...,w^L]$, then the max server utilization can be bounded by $\beta^{*}$. 
Otherwise, we could find a $w^{'}$ in the convex hull, such that the distance between $w$ and $w^{'}$ is minimized. We can view $w$ as a workload vector bursted on top of $w^{'}$.
Assume that the workload at a base station $B_m$ increases by a percentage of $\gamma$, i.e., $w_m=w_m^{'}(1+\gamma)$.
Then, if we load balance the additional workload $w_m^{'} \gamma$ uniformly among all the edge servers at base stations $B_n\in\Omega_m$ (other workloads are load balanced based on the service scheduling ratio computed by (\ref{eqn:calculateu})), then the maximum server utilization will be upper bounded by
$\beta^*+\frac{w_m^{'} \gamma}{\sum_{n\in \Omega_m}S^*_m}\leq \beta^*+\frac{\gamma}{\eta^*}$. Certainly, if we only solve (\ref{formulation:server_placement}) to obtain a server placement solution, we can still compute a resource pooling factor. However, this resource pooling factor can be much smaller than the optimal value $\eta^*$. As a result, the maximum server utilization can be much higher in case of workload burst. When the maximum server utilization is above one, some workload would be rejected.


%\noindent\textbf{Remark on Resource Pooling:} $\sum_{n\in \Omega_m(\delta)}S_m$ actually has a concrete physical meaning, which is the size of the \emph{resource pool} of the workload at the base station $B_m$. This robustification step is in fact trying to maximize the resource pools for all the workloads at different base stations. Readers may wonder why we do not use robust optimization to deal with the workload uncertainty. The reasons are two fold: 1) robust optimization has much higher computational complexity; 2) robust optimization yields poorer performance than our approach (see \S\ref{}).

\subsection{Reduce Algorithmic Complexity for Server Placement}
\label{sec:reducec_algorithmic_complexity}
We compute server placement results by solving (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}). However, both (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}) are integer programming problems, which are computationally expensive. In fact, we have tried solving (\ref{formulation:server_placement_robustification}) directly based on the Shanghai Telecom dataset with 3042 base stations, but unfortunately the state-of-the-art integer programming solver, Gurobi~\cite{gurobi}, cannot finish with a solution even after running a few hours.

To reduce computational complexity, we adopt a \emph{relaxing and rounding} approach. Specifically, we first allow the server placement variables $S$ to take fractional values. Then, both (\ref{formulation:server_placement})\footnote{The constraints (\ref{eqn:server_capacity}) contains a multiplicity term $S_n\beta$. To convert (\ref{formulation:server_placement}) into a linear programming problem, we need to substitute $S_n$ by $\hat{S}_n=S_n\beta$ in (\ref{eqn:server_capacity}), and replace (\ref{eqn:total_servers}) by $\sum_{m=1}^M \hat{S}_n = K\beta$ in (\ref{formulation:server_placement}).} and (\ref{formulation:server_placement_robustification}) can be converted to linear programming problems, which can be solved in polynomial time. After obtaining a fractional server placement solution of $S$, we can then round the fractional solution to an integer solution. Note that we need to ensure that (\ref{eqn:total_servers}) is satisfied after rounding.

Let $\tilde{S}^*=[\tilde{S}_1^*,\tilde{S}_2^*,...,\tilde{S}_M^*]$ be a fractional server placement solution. We have tried different rounding schemes as follows:
\begin{enumerate}
    \item \textbf{Smallest Resource Pool First (SRPF):} Each base station $B_m$ has a resource pool, whose size is $\sum_{B_n\in\Omega_m}\tilde{S}_n^*$. The base stations with smaller resource pools are given higher priority to round up its fractional solution.
    \item \textbf{Random Rounding (RR):} Randomly select some base stations to round up their fractional server counts.
    \item \textbf{Largest Resource Pool First (LRPF):} Contrary to the Smallest Resource Pool First policy, the base stations with larger resource pools are given higher priority to round up its fractional solution.
    \item \textbf{Largest Decimal First (LDF)}: The base stations with larger decimal part ($\tilde{S}_m^*-\lfloor \tilde{S}_m^*\rfloor$) are given higher priority to round up their fractional server counts.
    \item \textbf{Largest Scale-down First (LSF)}: When we round down a number $\tilde{S}_m^*$, the server placement solution is scaled down by $\frac{\tilde{S}_m^*-\lfloor \tilde{S}_m^*\rfloor}{\tilde{S}_m^*}$. The base stations with larger scale-down values are given higher priority to round up.
    %\item \textbf{Min Cost Flow Rounding}:Based on the Min Cost Flow Algorithm (Graph algorithm), we set the proportion between the decimal part of fractional solution and the fractional solution as the cost to get the integer results considering placing more servers to the area where the decimal part of servers weighs more. 
    %\item \textbf{Decimal Weight First}:Similar to the idea of Min Cost Flow Algorithm, we are inclined to round up the fractional solution  decimal part of which weighs more to the solution.
\end{enumerate}

Eventually, We adopt the Smallest Resource Pool First approach to perform rounding. This approach is the most robust against workload uncertainty, and our simulation results in Section \ref{sec:evaluate_rounding} further show that this approach yields the lowest workload rejection rate under bursty workload. 

%We briefly describe its intuition here. Consider a base station $B_m$ with a large resource pool. When the workload $w_m$ bursts, if the nearby BSs $B_n\in\Omega_m$ do not have enough resources, we can make room for $w_m$ by migrating other BSs' workload outside of the edge servers in $\Omega_m$. In Fig.~\ref{fig:motivation_dense}, three base stations(A, B and C) can provide resources to each other, belonging to resource-pools-dense area. Assume that the resource allocation units of base stations A and B is 7.8 firstly. With the help of resource pooling, even if we round them down, each base station can handle 8 units of workload.

%In contrast, if this base station $B_m$ is located in a resource-pools-sparse area, it might be hard for other BSs to make a room for $B_m$, and thus deploying more servers would help. In Fig.~\ref{fig:motivation_sparse}, D and E base stations are located in resource-pools-sparse area. Assume that the resource allocation units of base stations D and E is 7.1 firstly. without the help of resource pooling, only by rounding up can base station E handle 8 units of workload. on the contrary, base station D cannot handle it by rounding down.


% \begin{figure}[!htb]
%     \centering
%     \subfigure[Resource-pools-dense area.] {
%         \label{fig:motivation_dense}
%         \includegraphics[width=0.46\columnwidth]{images/motivation_dense.pdf}
%     }
%     \subfigure[Resource-pools-sparse area.] {
%         \label{fig:motivation_sparse}
%         \includegraphics[width=0.46\columnwidth]{images/motivation_sparse.pdf}
%     }
% \caption{Intuition example of Sparse-area First.}
% \label{fig:sparse-area_first}
% \end{figure}



\section{Server Scheduling}
When service providers deploy edge servers, they must ensure that there are enough servers even during peak hours. However, edge workloads exhibit strong diurnal pattern (see Figure~\ref{fig:traffic_demands}). Then, during idle hours, these edge servers may incur significant energy consumption unnecessarily, thus increasing the cost of edge computing.

To reduce cost, we study how to dynamically adjust the number of active servers based on the time-varying workload. When workload is low, we turn off some servers (or change to power saving mode) to save energy; when workload becomes higher, we will turn on some servers. 

We perform server on-off scheduling on daily basis. Specifically, We divide a day into $N$ equal-length time intervals $T=\{t_1,t_2,...,t_N\}$, where $t_n$ is the timestamp of the middle point of the $n$-th interval. At the day-ahead planning stage, we first predict the average workload vector $\bar{w}(t_n)=[\bar{w}_1(t_n), \bar{w}_2(t_n),...,\bar{w}_M(t_n)]$ in each time interval $t_n$ based on historical traces, and then compute a server on-off schedule for the following day.

\subsection{Server Scheduling without Considering Switching Cost}
We first ignore the switching cost of toggling servers between on/off states. Then, we can study server scheduling in each time interval separately. In this case, the server scheduling problem becomes very similar to the server placement problem, and thus the methodology used in Section \ref{sec:server_placement} can be also applied here. The only difference is that we only need to account for one workload vector in server scheduling.

Let $K(t)$ be the total number of active servers at time $t$. Then, the number of active servers $S(t)=[S_1(t),S_2(t),...,S_M(t)]$ at time $t$ must satisfy (\ref{eqn:active_servers}) as well as the following constraint:
\begin{equation}\label{eqn:scheduling_server_num}
    \sum_{m=1}^M S_{m}(t) = K(t).
\end{equation}
Let $\beta(t)$ be the maximum server utilization at time $t$ and $u(t) = [u_{mn}(t),m,n = 1,2,...,M]$ be the service scheduling variables satisfying (\ref{eqn:demand_split}). Then, we can convert  (\ref{eqn:server_capacity}) to
\begin{equation}\label{eqn:scheduling_capacity}
\sum_{m=1}^M \bar{w}_m(t) u_{mn}(t)\leq S_n(t) C \beta(t).
\end{equation}
Let $\eta(t)$ be the resource pooling factor at time $t$. Then, the constraint (\ref{eqn:resource_pool_factor}) can be rewritten as
\begin{equation}\label{eqn:scheduling_resource_pool_factor}
    \eta(t) \bar{w}_m \leq \sum_{B_n\in \Omega_m}S_n(t).
\end{equation}

Then, we can compute a server scheduling solution at time $t$ in two steps:

\noindent\textbf{Step 1:} Compute the optimal $\beta^*(t)$ by solving
\begin{equation}\label{formulation:server_scheduling_no_switching_cost_step1}
\boxed{
\begin{aligned}
\min_{S(t),u(t),\beta(t)} & \hspace{20mm}\beta(t) &\\
\text{s.t.}\hspace{5mm}& S(t),u(t),\beta(t)\text{ satisfy (\ref{eqn:demand_split})(\ref{eqn:active_servers})(\ref{eqn:scheduling_server_num})(\ref{eqn:scheduling_capacity}).}&
\end{aligned}
}
\end{equation}
\noindent\textbf{Step 2:} Compute the optimal $S^*(t)$ and $\eta^*(t)$ by solving
\begin{equation}\label{formulation:server_scheduling_no_switching_cost_step2}
\boxed{
\begin{aligned}
\max_{S(t),u(t),\eta(t)} & \hspace{20mm}\eta(t) &\\
\text{s.t.}\hspace{6mm}& \hspace{-3mm}S(t),u(t),\beta^*(t),\eta(t)\text{ satisfy (\ref{eqn:demand_split})(\ref{eqn:active_servers})(\ref{eqn:scheduling_server_num})(\ref{eqn:scheduling_capacity})(\ref{eqn:scheduling_resource_pool_factor}).}&
\end{aligned}
}
\end{equation}

Clearly, for different $K(t)$, we can obtain different solutions of $S^*(t)$. To understand how many active servers are required, we use historical traces to calculate the fraction of rejected workload. From Fig.~\ref{fig:draw_server_scheduling_error_workload2}, we can see that different number of active servers are required to ensure low workload rejection rate. Specifically, the workload between time 0:00 and 1:00 is low, and thus approximately 4500 servers are sufficient to offer close-to-zero workload rejection rate. In contrast, the workload at 08:00-09:00, 12:00-13:00 and 21:00-22:00 is much higher, thus requiring more active servers.

Based on the above analysis, we can pick a $K^*(t)$ that leads to close-to-zero workload rejection rate for each time interval $t$, and then use $K^*(t)$ to compute $S^*(t)$.

%As shown in Fig.(\ref{fig:draw_server_scheduling_error_workload2}), we statistic the rejected workload in four different time slots as the increase of the number of servers. It is obvious that the four curves converge at different point. In Fig.(\ref{fig:draw_server_scheduling_error_workload2}), we divide a day into 24 time slots and 1 hour for a slot. $time_0$ means the time between 0:00 and 1:00 which clearly has fewer user requests and the curve to $time\_0$ converges at small amount of servers, approximately 4500. What's more, in the time slot with more user demands like $time\_12$ and $time\_21$, the curve may converge at the number of 7000.Therefore, according to the experiment based on the real user demands, we can make sure activating fixed number of servers for each time slot will not influence the service quality to some extent.

%In each time slot, in our formulation, as equation.(\ref{eqn:scheduling_server_num}) shown, we can set a fixed number of servers $K(t)$ for each time slot due to the diurnal patterns proved in Figure (\ref{fig:traffic_demands}) (\ref{fig:requests_duration}) (\ref{fig:requests_inter_arrival}) . We want to make sure if we can get a proper and efficient $K(t)$ with fewer rejected events.

%Therefore, based on the real user demands and server scheduling formulation(\ref{formulation:server_scheduling})(\ref{formulation:server_placement_robustification}) with Sparse-area Fist rounding scheme we use, we analyze the changes of the number of failed events with the increase of the server number used in the our server scheduling model.

\begin{figure}[!htb]
    \centering
    % \includegraphics[width=0.8\linewidth]{images/draw_scheduling_error_server_plot.pdf}
    \includegraphics[width=0.8\linewidth]{images/draw_server_scheduling_error_workload2.pdf}
    \caption{Workload rejection rate under different number of servers in different periods.}
    \label{fig:draw_server_scheduling_error_workload2}
\end{figure}

\subsection{Considering Switching Cost for Server Scheduling}
We account for the switching cost for server scheduling in this section. To ensure close-to-zero workload rejection rate, we slightly modify the constraint (\ref{eqn:scheduling_server_num}) as
\begin{equation}\label{eqn:scheduling_server_num_guarantee}
    \sum_{m=1}^M S_{m}(t) \geq K^*(t).
\end{equation}
When $K(t)=K^*(t)$, we can solve (\ref{formulation:server_scheduling_no_switching_cost_step1}) and (\ref{formulation:server_scheduling_no_switching_cost_step2}) to obtain $\beta^*(t)$ and $\eta^*(t)$ first. Then, we can modify (\ref{eqn:scheduling_capacity}) and (\ref{eqn:scheduling_resource_pool_factor}) as
\begin{equation}\label{eqn:scheduling_capacity_guarantee}
\sum_{m=1}^M \bar{w}_m(t) u_{mn}(t)\leq S_n(t) C \beta^*(t).
\end{equation}
\begin{equation}\label{eqn:scheduling_resource_pool_factor_guarantee}
    \eta^*(t) \bar{w}_m \leq \sum_{B_n\in \Omega_m}S_n(t).
\end{equation}

Then, we can compute a server scheduling solution by minimizing the cost function (\ref{eqn:cost}) as follows:
\begin{equation}\label{formulation:server_scheduling}
\boxed{
\begin{aligned}
&\hspace{-5mm}\textbf{Server On-off Scheduling:}&\\
\min_{S(t)} & \hspace{2mm}\sum_{m=1}^M\sum_t\bigg(E_r S_m(t) + E_s(S_m(t)-S_m(t-1))^+\bigg) &\\
\text{s.t.}\hspace{1mm}& \hspace{2mm}S(t),u(t)\text{ satisfy (\ref{eqn:demand_split})(\ref{eqn:active_servers})(\ref{eqn:scheduling_server_num_guarantee})(\ref{eqn:scheduling_capacity_guarantee})(\ref{eqn:scheduling_resource_pool_factor_guarantee}) for any }t.&
\end{aligned}
}
\end{equation}
Note that the term ``$E_s(S_m(t)-S_m(t-1))^+$'' captures the switching cost.

\noindent\textbf{Remark: } We need to solve (\ref{formulation:server_scheduling_no_switching_cost_step1}) and (\ref{formulation:server_scheduling_no_switching_cost_step2}) multiple times to obtain $K^*(t),\beta^*(t)$ and $\eta^*(t)$ before solving (\ref{formulation:server_scheduling}). This pre-solving step is critical to ensure low workload rejection rate.

\noindent\textbf{Remark on Algorithmic Complexity:} Although server on-off scheduling is only calculated once everyday, directly solving (\ref{formulation:server_scheduling_no_switching_cost_step1}), (\ref{formulation:server_scheduling_no_switching_cost_step2}) and (\ref{formulation:server_scheduling}) is still computationally prohibitive. To reduce complexity, we can adopt the same \emph{relaxing and rounding} approach proposed in Section \ref{sec:reducec_algorithmic_complexity}.

%Based on the result of formulation (\ref{formulation:server_scheduling}) and formulation (\ref{formulation:server_scheduling_robustification}), we can get the fractional solution of every time slot.Naturally, we need to transform all fractional results into integer ones. Based on the analysis in \ref{sec:reducec_algorithmic_complexity}, the Sparse-area First result can also be applied in the server scheduling schemes.


% Recall that we have adopted a two-step approach for server placement.
% We divide a day into $N$ equal-length time slots $T=\{t_1,t_2,...,t_N\}$, where $t_n$ is the . Given several sequences based on different time slots of historical workload vectors, we can easily acquire an average workload metrix, represented by $w_{s} = \{w_{m}(t),m = 1,2,\cdots,M, t = T_{1},T_{2},\cdots,T_{N}\}$.Note that $w_{s}$ is time-variant considering server on-off scheduling is adjusted based on the recent service conditions.

% Making sure the server placement schemes $S_{m}$, we optimize the scheduling variable $S(t)=[S_m(t),m=1,2,...,M]$ satisfying (\ref{eqn:active_servers}).Considering the difference between workload at idle and busy time, we control certain number of servers,noted by $K(t)$ to be activated at certain time:

% Considering the strong diurnal pattern of user requests, in the same time slot of each day, we can activate the same number of servers under the condition that we can maintain the service quality.

% Similar to the server placement model, we also optimize the service placement variable $u = [u_{mn}(t),m,n = 1,2,\cdots,M]$ satisfying(\ref{eqn:demand_split}).therefore, we can transfer 

% We still use $\beta$ to restrict the edge server utilization to guarantee better server quality and our scheduling formulation can be  presented as:



% This scheduling formulation is under our data analysis that the user requests to the servers have strong diurnal pattern and in the same time slot, the real-time workload is similar to the historical workload and the same number of servers can function well all the time.


% \subsection{Handling Demand Uncertainty}
% In \ref{sec:resource_pooling}, we introduce the resource pooling idea and use it to reduce the rejected events led by the workload uncertainty. Considering the similarity between our server placement scheme and server scheduling idea, especially in the condition shown in Fig.\ref{fig:motivation}. So we also use resource pooling idea to reduce the rejected events resulted by the demand uncertainty.

% Similarly, we still maximize the resource pooling factor $\eta$ which in each time slot satisfying:

% Then, we can give the resource pooling formulation in server scheduling condition:

% Note that $\beta^*$ is the optimal value of the formulation (\ref{formulation:server_scheduling}). Thus, before solving (\ref{formulation:server_scheduling_robustification}), we need to solve (\ref{formulation:server_scheduling}) first.






==> IWQoS2021(Extended)/sections/6Implementation.tex <==
\section{Deployment Details}
This section may not be necessary, just like the other MEC papers.

\subsection{Hardware Interconnection}

\subsection{Software Control}
Describe the software architecture and control ideas needed.

With the help of Cloudlet?

\section{A Close-to-Optimal Algorithm for Server Placement with Polynomial Complexity}
We compute a server placement solution in two steps: 1) ignore the integer requirement on $[S_m]$, and compute a fractional solution first; 2) round the fractional solution of $[s_m]$ to an integer solution using min cost flow.

\subsection{Compute a Fractional Solution}
After removing the integer requirement on $[S_m]$, it is easy to check that (\ref{formulation:server_placement_robustification}) becomes a linear problem problem, which can be solved in polynomial time. However, (\ref{formulation:server_placement}) becomes a bi-linear problem (the constraints (\ref{eqn:server_capacity}) contain a multiplication term between the variables $S_{m}$ and $\beta$), which is still hard to solve. 

Fortunately, (\ref{formulation:server_placement}) can be easily transformed to an linear problem using the following variable substitution:
\begin{equation}\label{eqn:variable_substitution}
u_{mn}^{'} = \frac{u_{mn}w_m}{C\beta}, \kappa = \frac{1}{C\beta}.
\end{equation}
Using $u_{mn}^{'}$ and $\kappa$, the constraints (\ref{eqn:demand_split}) and (\ref{eqn:server_capacity}) are transformed into
\begin{equation}\label{eqn:demand_split_new}
u_{m1}^{'}+u_{m2}^{'}+\cdots+u_{mM}^{'}=w_m\kappa, m=1,2,...,M,
\end{equation}
\begin{equation}\label{eqn:server_capacity_new}
u_{1n}^{'}+u_{2n}^{'}+\cdots+u_{Mn}^{'} \leq S_{n}, n=1,2,...,M.
\end{equation}
The original optimization problem (\ref{formulation:server_placement}) is now transformed into:
\begin{equation}\label{formulation:server_placement_new}
\boxed{
\begin{aligned}
\max_{S_m,u_{mn}^{'},\kappa} & \hspace{20mm}\kappa &\\
\text{s.t.}& \hspace{3mm} S_m,u_{mn}^{'},\kappa\text{ satisfy (\ref{eqn:demand_split_new})(\ref{eqn:total_servers})(\ref{eqn:server_capacity_new})}&\\
&\hspace{3mm}0\leq u_{mn}^{'}\leq w_m\kappa\text{ and } u_{mn}^{'}=0\text{ for }n\notin \Omega_{m}(\delta) &
\end{aligned}
}
\end{equation}
Clearly, if we ignore the integer requirement on $[S_m]$, (\ref{formulation:server_placement_new}) becomes a linear programming problem.

% \begin{equation}
% 	\left\{ 
% 	\begin{array}{c}
% 	u_{11}^{'}(t)+u_{12}^{'}(t)+u_{13}^{'}(t)+\cdots+u_{1M}^{'}(t) = 1/\beta \\ 
% 	u_{21}^{'}(t)+u_{22}(t)+u_{23}^{'}(t)+\cdots+u_{2M}^{'}(t) = 1/\beta  \\ 
% 	\cdots\cdots\cdots\cdots  \\
% 	u_{M1}^{'}(t)+u_{M2}(t)+u_{M3}^{'}(t)+\cdots+u_{MM}^{'}(t) = 1/\beta  \\ 
% 	\end{array}
% 	\right. 
% \end{equation}
% \begin{equation}
% \left\{ 
% \begin{array}{c}
% u_{11}^{'}(t)w_1(t)+u_{21}^{'}(t)w_2(t)+\cdots+u_{M1}^{'}(t)w_M(t) \leq S_{1}*C \\ 
% u_{12}^{'}(t)w_1(t)+u_{22}^{'}(t)w_2(t)+\cdots+u_{M2}^{'}(t)w_M(t) \leq S_{2}*C  \\ 
% \cdots\cdots\cdots\cdots  \\
% u_{1M}^{'}(t)w_1(t)+u_{2M}^{'}(t)w_2(t)+\cdots+u_{MM}^{'}(t)w_M(t) \leq S_{M}*C  \\ 
% \end{array}
% \right. 
% \end{equation}

\subsection{Round the Fractional Solution to An Integer Solution}
Let $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}, \tilde{\eta}$ be the fractional server placement solution obtained from solving (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}) as linear programming problems. Since we have relaxed the integer requirement of $S_m$, the resulting $\tilde{\beta}$ must be a lower bound of the optimal value of (\ref{formulation:server_placement}), while $\tilde{\eta}$ must be an upper bound of the optimal value of (\ref{formulation:server_placement_robustification}). In order to convert the fractional solution to an integer solution, we first introduce some mathematical preliminaries on the min cost circulation problem.

\subsubsection{Mathematical Preliminaries on the Min Cost Circulation Problem}
\begin{definition}\label{mincostcirculation}
(Min-Cost Circulation Problem) Given a flow network with
\begin{itemize}
  \item $l(v,w)$, lower bound on flow from node $v$ to node $w$;
  \item $u(v,w)$, upper bound on flow from node $v$ to node $w$;
  \item $c(v,w)$, cost of a unit of flow on $(v,w)$,
\end{itemize}
the goal of the min-cost circulation problem is to find a flow assignment $f(v,w)$ that minimizes
$$\sum_{(v,w)}c(v,w)\cdot f(v,w),$$
while satisfying the following two constraints:
\begin{enumerate}
  \item Throughput constraints: $l(v,w)\leq f(v,w)\leq u(v,w)$;
  \item Flow conservation constraints: $\sum_u f(u,v) = \sum_w f(v,w)$ for any node $v$.
\end{enumerate}
\end{definition}

Note that all the constant parameters $l(v,w),u(v,w)$ are all positive and $c(v,w)$ can be either positive or negative. In addition, min-cost circulation problem has a very nice property that guarantees integer solutions:
\begin{lemma}\label{integralflowtheorem}
(Integral Flow Theorem) Given a feasible circulation problem, if $l(v,w)$'s and $u(v,w)$'s are all integers, then there exists a feasible flow assignment such that all flows are integers.
\end{lemma}

In fact, for feasible circulation problems with integer bounds, most max-flow algorithms, e.g., Edmonds-Karp algorithm \cite{Edmonds1972Theoretical} and Goldberg-Tarjan algorithm \cite{Goldberg1988A}, are guaranteed to generate integer solutions.

\subsubsection{Mapping the Server Placement Problem to a Min Cost Circulation Problem}

We would like to find an integer solution for $S_m$ satisfying (\ref{eqn:demand_split})(\ref{eqn:total_servers})(\ref{eqn:server_capacity}) around the fractional solution $\tilde{S}_m$. The basic idea is to map these constraints to the flow conservation constraints in the min cost circulation problem. 

\noindent\textbf{Step 1:} Let $\tilde{u}_{mn}^{'} = \frac{\tilde{u}_{mn}w_m}{C\tilde{\beta}}$ and $\tilde{\kappa}=\frac{1}{C\tilde{\beta}}$. We first prove that $\tilde{u}_{mn}^{'}$ and $\tilde{S}_m$ satisfy
\begin{subequations}
\begin{align}
    &\tilde{u}_{m1}^{'}+\tilde{u}_{m2}^{'}+\cdots+\tilde{u}_{mM}^{'}=w_m\tilde{\kappa}, \hspace{3mm}m=1,2,...,M;\label{subeqn:demand_split}\\
    &\tilde{u}_{1n}^{'}+\tilde{u}_{2n}^{'}+\cdots+\tilde{u}_{Mn}^{'}=\tilde{S}_n, \hspace{3mm}n=1,2,...,M;\label{subeq:capacity}\\
    &\tilde{S}_1+\tilde{S}_2+\cdots+\tilde{S}_M=K.\label{subeq:num_servers}
\end{align}
\end{subequations}
(\ref{subeqn:demand_split}) and (\ref{subeq:num_servers}) follow directly from the constraints (\ref{eqn:demand_split}) and (\ref{eqn:total_servers}). However, for (\ref{subeq:capacity}), the constraint (\ref{eqn:server_capacity}) only implies
$$\tilde{u}_{1n}^{'}+\tilde{u}_{2n}^{'}+\cdots+\tilde{u}_{Mn}^{'}\leq \tilde{S}_n.$$
To see why equality holds in (\ref{subeq:capacity}), we use the fact that $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}$ is actually an optimal fractional solution of (\ref{formulation:server_placement}). If the equality in (\ref{subeq:capacity}) does not always hold, we can reduce $\tilde{S}_m$ to $\tilde{S}_m^{'}$ to make the equality in (\ref{subeq:capacity}) hold. In this case, we must have $$\tilde{S}_1^{'}+\tilde{S}_2^{'}+\cdots+\tilde{S}_M^{'}<K.$$
Let $\rho = \frac{\sum_{n=1}^M \tilde{S}_n^{'}}{K}<1$, then it is easy to check that $\frac{1}{\rho}\tilde{S}_m^{'}, \tilde{u}_{mn}, \rho\tilde{\beta}$ is also a feasible fractional solution of (\ref{formulation:server_placement}). However, $\rho\tilde{\beta}<\tilde{\beta}$, which contradicts to the fact that $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}$ is an optimal solution of (\ref{formulation:server_placement}).


\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.44]{./images/min_cost_flow.pdf}
    \caption{The flow graph corresponding to (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}).}
    \label{fig:min_cost_flow}
\end{figure}

\noindent\textbf{Step 2:}
Based on the constraints (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}), we construct a flow graph as follows (also see Fig. \ref{fig:min_cost_flow}):
\begin{enumerate}
  \item Create a directed $M\times M$ bipartite graph. We create $M$ nodes on the left hand side of the bipartite graph, and create $M$ nodes on the right hand side of the bipartite graph. We add a directed link from $m$ to $n$, and set the bounds of this link as $[\lfloor \tilde{u}_{mn}^{'}\rfloor, \lceil\tilde{u}_{mn}^{'}\rceil]$ and the cost of this link as $0$.
  \item Add a source node, $M$ directed links for this source node to the $M$ left nodes. The bounds of the $m$-th link is set as $[\lfloor w_m\tilde{\kappa} \rfloor, \lceil w_m\tilde{\kappa}\rceil]$, and the cost is set to 0. %$\frac{\lfloor w_m\tilde{\kappa} \rfloor}{w_m\tilde{\kappa}}$.
  \item Add a sink node and $M$ directed links from the $M$ right nodes to this sink node. The bounds of the $m$-th link is set as $[\lfloor \tilde{S}_m \rfloor, \lceil \tilde{S}_m\rceil]$, and the cost is set to $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$.
  \item Add a feedback link from the sink node to the source node. The bounds of this feedback link is set as $[K,K]$, and the cost is set to $0$.
\end{enumerate}
In this flow graph, the flow conservation constraint on each left node corresponds to one of the constraints in (\ref{subeqn:demand_split}); the flow conservation constraint on each right node corresponds to one of the constraints in (\ref{subeq:capacity}); and the flow conservation constraint on the sink node corresponds to the constraint (\ref{subeq:num_servers}). Hence, according to (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}), it is easy to construct a feasible flow assignment for the above flow graph as follows:
\begin{enumerate}
    \item Assign $w_m\tilde{\kappa}$ amount of flow to the link between the source node and the $m$-th left node;
    \item Assign $\tilde{u}_{mn}^{'}$ amount of flow to the link between the $m$-th left node and the $n$-th right node;
    \item Assign $\tilde{S}_m$ amount of flow to the link between the $n$-th right node and the sink node;
    \item Assign $K$ amount of flow to the link between the sink node and the source node.
\end{enumerate}

Since all the bounds in the above flow graph are integers, according to Lemma \ref{integralflowtheorem}, this flow graph must have an integer solution with the minimum cost, which can be computed in polynomial time using algorithms like, Edmonds-Karp algorithm~\cite{Edmonds1972Theoretical} and Goldberg-Tarjan algorithm~\cite{Goldberg1988A}. In our own implementation, we have used Google OR-Tools~\cite{OrTools} as our min cost circulation problem solver. After obtaining an integer flow assignment for the above min cost circulation problem, the flow values of the $M$ links between the right nodes and the sink node give the server placement results, which we denote by $[S_1^*,S_2^*,...,S_M^*].$

\noindent\textbf{Remark on the unit cost:} Note that we set the unit cost of the link between the $m$-th right node and the sink node as $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$. The reason is that we want to minimize the rounding loss. $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$ can be interpreted as the remaining fraction of capacity after rounding down. If this number is small, we should try to avoid rounding down. This step is critical for our min cost circulation based approach to achieve close to optimal performance.

\noindent\textbf{Remark on the optimality:} Rigorously speaking, the min cost flow based approach is not optimal. However, as the edge workload increases, more servers will be deployed. As a result, the values of $\tilde{S}_m$ become large, and  $S_m^*/\tilde{S}_m$ approaches to 1 because $S_m^*\in [\lfloor \tilde{S}_{m}\rfloor, \lceil\tilde{S}_{m}\rceil]$. As $S_m^*/\tilde{S}_m$ approaches to 1, the objective values of (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}) also approach the performance bound $\tilde{\beta}$ and $\tilde{\eta}$.

\noindent\textbf{Versus native rounding approaches:} Our min cost circulation based rounding approach seems complicated. Readers may question the necessity of using such a approach. In fact, before proposing this min cost circulation based rounding approach, we have tried some naive rounding approaches. However, these rounding approaches exhibit poor performance (see \S\ref{}).

% \noindent\textbf{Step 3: Understanding the Performance Gap.} The essence of the min cost flow based approach is to imitate the fractional solution as much as possible. That is why we expect it to have close-to-optimal performance in practice. Next, we provide some theoretical analysis on its performance. We also conduct numerical analysis in \S\ref{}.

% Let $S_m^*, u_{mn}^*, \beta^*, \eta^*$ be the optimal server placement solution obtained by solving (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}).
% Let $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}, \tilde{\eta}$ be the optimal fractional server placement solution, and let $S_m^{**}, u_{mn}^{**}, \beta^{**}, \eta^{**}$ be the server placement solution obtained using the min cost circulation based approach. 


%For the server placement model and server scheduling model ,considering the number of servers $S_{n}$  and the number of operating servers $S_{n}(t)$ in AP $A_{n}$ are all integers, we use integer programming to solve the problem. But integer programming has high complexity which may consume lots of time to get the solution. As a consequence, considering the linear programming's low complexity, we decide to transfer 

% We prove the following theorem:
% \begin{theorem}\label{thm:circulation}
% Consider the following ILP:
% \begin{eqnarray}\label{eqn:general_form}
% &\min\limits_{\mathbf{a}=[a_{ij}]}& \sum_{i=1}^I\sum_{j=1}^J C_{ij}a_{ij}\\
% &\text{s.t.}&A_{ij}^L \leq a_{ij} \leq A_{ij}^U, \quad \forall \; i,j=1,...,N,\nonumber\\
% &&P_j^L\leq \sum_{i=1}^I a_{ij}\leq P_j^U,\quad \forall \; j=1,...,N,\nonumber\\
% &&Q_i^L\leq \sum_{j=1}^J a_{ij}\leq Q_i^U,\quad \forall \; i=1,...,N,\nonumber
% \end{eqnarray}
% where ${\bf a}=[a_{ij}]$ is an $I\times J$ matrix, and ${\bf C}=[C_{ij}], {\bf P}^L=[P_j^L], {\bf Q}^L=[Q_i^L], {\bf P}^U=[P_j^U], {\bf Q}^U=[Q_i^U], {\bf A}^L=[A_{ij}^L], {\bf A}^U=[A_{ij}^U]$ are integer constants. (Note that ${\bf C}=[C_{ij}]$ can be negative.) If (\ref{eqn:general_form}) has a fractional solution, then (\ref{eqn:general_form}) must have an integer solution, which can be solved in polynomial time.
% \end{theorem}

==> IWQoS2021(Extended)/sections/7Evaluation.tex <==
\section{Evaluation}
\subsection{Introduce the Trace for Evaluation}
\subsubsection{Shanghai Telecom's Real Communication Records}
We have introduced this real trace in Section \ref{sec:workload_analysis}. This trace contains communication records for 3042 base stations and 6236620 user requests over a time span of six months. We will use this trace to compare our server placement and server scheduling solution against previous approaches. 

%It is also used for calculating the least servers we need to use with least cost and best service quality.\\

\subsubsection{Synthetic Trace}
It was shown in Section \ref{sec:workload_observation3} that edge workload is hard to predict accurately. Hence, our solution must be robust against potential workload bursts. Unfortunately, the historical real traces may not offer a comprehensive coverage over the burst patterns. Hence, we construct synthetic traces to evaluate solution robustness.

Our synthetic traces are constructed as follows. Given an arbitrary real workload vector $w=[w_1,w_2,...,w_M]$, we randomly select a set  containing 100-200 BSs out of the 3024 BSs, choose a scaling factor in $\{1.2, 1.5, 1.8, 2\}$ and then scale up the workload of all the selected BSs by this scaling factor. For the same real workload vector, we repeat the above step multiple times and generate a total of 240 bursty workload vectors. Note that we generate workload bursts by multiplying the original workload by a scaling factor. The reason is that the workload with the highest variability has its standard deviation scaling approximately linearly with respect to its average value (see Fig. ~\ref{fig:traffic_delta:b} in Section \ref{sec:workload_analysis}).

%Synthetic trace is the trace that we randomly add unexpected events to the real trace. We use the synthetic trace to compare the robustness of different detailed methods in our formulation.

%1.2 1.5 1.8 2; 100; one future workload vector.

\subsection{Compare Different Server Placement Policies}\label{sec:compare_server_placement}
We group existing server placement policies into three categories and evaluate them using the real trace.

\noindent\textbf{Traffic-agnostic policies}: This policy does not use any workload information for server placement. We evaluate the following policies in this category:
\begin{enumerate}
\item \textbf{Random}: Place $K$ servers at randomly chosen BSs.

\item \textbf{Clustering}: Use k-means algorithm to group BSs into $k$ clusters. Let $s_i^{(C)}$ be the number of BSs in the $i$-th cluster. Place $K\frac{s_i^{(C)}}{\sum_{i=1}^k s_i^{(C)}}$ servers at the centroid of the $i$-th cluster.

\item \textbf{Uniform}: Divide the geographical area into fixed-sized zones. Let $s_i^{(U)}$ be the number of BSs in the $i$-th zone. Place $K\frac{s_i^{(U)}}{\sum_{i=1}^k s_i^{(U)}}$ servers at the centroid of the $i$-th zone.
\end{enumerate}

\noindent\textbf{Traffic-aware but uncertainty-agnostic policies}: This policy computes server placement based on a predicted workload vector, but does not account for the workload uncertainty. We evaluate two policies in this category:
\begin{enumerate}
\item \textbf{Traffic-aware without load balancing (TwithoutLB)}: In this policy, the workload at each BS can be only allocated to the nearest BS with edge servers. Many existing server placement policies fall into this category~\cite{Wang2019Edge, Guo2019User,Zeng2018Edge,Li2018An,Chin2020Queuing,Cao2020Exploring, Kasi2020Heuristic, Ren2018A, guo2020user}. In this paper, we use k-means algorithm to group BSs into $k$ clusters, and assign all the workload in each cluster to the centroid of this cluster. Let $l_i$ be the total workload of the BSs in the $i$-th cluster. Place $K\frac{l_i}{\sum_{i=1}^k l_i}$ servers at the centroid of the $i$-th cluster.

\item \textbf{Traffic-aware with load balancing (TwithLB)}: In this policy, the workload at each BS can be load balanced to the close-by BSs. This setting was also adopted in \cite{Tero2020Edge, Xu2016Efficient, Jia2017Optimal,Yang2019Cloudlet}. Here, we compute a server placement solution by solving (\ref{formulation:server_placement}) with only one workload vector. (We use historical average workload vector in the evaluation.)
\end{enumerate}

\noindent \textbf{Traffic and uncertainty-aware policies}: This is our server placement strategy proposed in Section \ref{sec:server_placement} (namely RO-RP).

%first use robust optimization based on multiple workload patterns, and then maximize the resource pool factor to make our solution robust to demand uncertainty.

% This policy accounts for both the workload pattern and uncertainty. We evaluate two policies in this category:
% \begin{enumerate}
% \item \textbf{Resource Pooling}: This is our proposed server placement strategy. By maximizing the resource pool factor, we make our traffic-aware server placement policy robust to demand uncertainty.

% \item \textbf{Robust Optimization}: To improve solution robustness to traffic uncertainty, we use multiple workload vectors to compute a server placement solution. The detailed formulation is given by (\ref{formulation:robust_optimization_server_placement}).
% \end{enumerate}

% \begin{enumerate}
% \item \textbf{random}: Place random number of servers in different base stations randomly. 800, [0,20]

% \item \textbf{K-means}: Use K-Means algorithm to decide the server placement scheme. 200.
% top-K

% \item \textbf{Uniform}: Place the servers uniformly at each base station. 8000/3000

% \item \textbf{ILP}: With our formulation, we use  integer programming to get the server placement results. No resource pooling.

% \item \textbf{LP +  Formulation}: With our formulation, we use  linear programming method and then use rounding approach Sparse-area First to get integer result .

% \item \textbf{Resource Pooling}: With our formulation, we use Resource Pooling under the result of linear programming. Then we get integer result by rounding approach Sparse-area First.
% \end{enumerate}

\begin{figure*}[!htb]
    \centering
    \subfigure[Workload rejection rate for six server placement policies.] {
        \label{fig:draw_history_compare_error}
        \includegraphics[width=0.64\columnwidth]{images/draw_history_compare_error.pdf}
    }
    \subfigure[A zoom in of the performance for the top-3 best server placement policies.] {
        \label{fig:draw_history_compare_error_b}
        \includegraphics[width=0.64\columnwidth]{images/draw_history_compare_error_b.pdf}
    }
    \subfigure[Number of servers required for the top-3 best server placement policies.] {
        \label{fig:draw_error_server_plot}
        \includegraphics[width=0.64\columnwidth]{images/draw_server_num_compare_error.pdf}
    }
\caption{Comparison of different server placement policies.}
\label{fig:diff_method_error}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \subfigure[Performance of different rounding schemes.] {
        \label{fig:overload_round_error_rate_cdf}
        \includegraphics[width=0.64\columnwidth]{images/overload_round_error_rate_cdf.pdf}
    }
    \subfigure[Average workload vs. component-wise max workload.] {
        \label{fig:overload_robust_balance_pool}
        \includegraphics[width=0.64\columnwidth]{images/overload_robust_balance_pool.pdf}
    }
    \subfigure[Contribution of robust optimization and resource pooling.] {
        \label{fig:overload_error_rate_cdf_80000}
        \includegraphics[width=0.64\columnwidth]{images/overload_error_rate_cdf_80000.pdf}
    }
\caption{Different design choices of our server placement policy.}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \subfigure[The switching cost is equal to running a server in idle state for one hour.] {
        \label{fig:draw_energy_consumption_1}
        \includegraphics[width=0.64\columnwidth]{images/draw_energy_consumption_1.pdf}
    }
    % \subfigure[0.5.] {
    %     \label{fig:draw_energy_consumption_05}
    %     \includegraphics[width=0.64\columnwidth]{images/draw_energy_consumption_05.pdf}
    % }
    \subfigure[The switching cost is equal to running a server in idle state for 12 minutes.] {
        \label{fig:draw_energy_consumption_02}
        \includegraphics[width=0.64\columnwidth]{images/draw_energy_consumption_02.pdf}
    }
    \subfigure[Benefit of accounting for switching cost explicitly.] {
        \label{fig:draw_energy_consumption_count}
        \includegraphics[width=0.64\columnwidth]{images/draw_energy_consumption_count.pdf}
    }
\caption{Evaluation of server scheduling.}
\label{fig:draw_energy_consumption}
\end{figure*}

% \begin{figure}[!htb]
%     \centering
%     % \includegraphics[width=0.8\linewidth]{images/draw_error_server_plot.pdf}
%     \includegraphics[width=0.2\linewidth]{images/draw_server_num_compare_error.pdf}
%     \caption{xxx.}
%     \label{fig:draw_error_server_plot}
% \end{figure}

%\subsubsection{Use synthetic trace}

%\subsubsection{Compare the number of required servers}
%Under the same request rejection ratio, how many servers can be saved with our solution?\\\noindent

We use two weeks of real traces to evaluate the workload rejection rate for different server placement policies. In Fig.~\ref{fig:diff_method_error}, we fix the total number of servers as 8000. Apparently, our approach achieves the lowest workload rejection rate. In Fig.~\ref{fig:draw_error_server_plot}, we vary the number of servers from 7000 to 12000, and study how many servers are required in order to achieve close-to-zero workload rejection rate. Under our policy, approximately 7500 servers are required. In contrast, the second best option requires about 10000 servers.

%we use the total number of failed events in each hour to evaluate the service quality and statistic the total failed events of half a month. Obviously, the service quality of our formulation is better than that of previous approaches. Among the methods used in our formulation, the Resource Pooling method has the best performance in service quality.

%As for Fig.~\ref{fig:draw_error_server_plot}, we use trends about the number of error events in the same time slot as the number of servers we are willing to place increases to evaluate the performance of our methods. Considering the cost, it is obvious the less servers we use when the number of error events converges to 0, the better our method is. Owing to the worst performance of the Random Formulation and K-Means Formulation, we mainly compare the other four methods with similar service quality. The Resource Pooling method uses less servers and have better performance.

\subsection{Understand Different Design Choices of RO-RP}
\subsubsection{Evaluating different rounding schemes}\label{sec:evaluate_rounding}
To reduce the computational complexity of integer programming, we use linear programming to obtain a fractional solution first and then use a rounding scheme to get an integer solution (see Section \ref{sec:reducec_algorithmic_complexity}). Therefore, the effects of different rounding schemes should be evaluated.

We use the synthetic trace to evaluate the workload rejection rate of different rounding schemes, because our synthetic trace has a better coverage over the potential bursts than the real trace. In Fig.~\ref{fig:overload_round_error_rate_cdf}, we evaluate all the rounding schemes proposed in Section \ref{sec:reducec_algorithmic_complexity}.
Evidently, The Smallest  Resource  Pool  First Scheme has the best performance. In contrast, the Largest Resource Pool First Scheme performs the worst. 

%Fig.~\ref{fig:round_compare_cdf} plots the CDF of the workload rejection rate. The closer the curve is to the upper left corner, the better the rounding scheme is.

%Therefore,it proves placing more servers to the area with less flows can achieve better effect.

%Due to the Randomness of Random Rounding Scheme, we evaluate two different results with the same Random Rounding Scheme.

%Considering different rounding schemes have similar performances on real trace, we use synthetic trace with more unexpected events to test the robustness of each scheme and  the CDF (Cumulative Distribution Function) to show the possibility of different number of failed requests in Fig.~\ref{fig:round_compare_cdf}. The closer the curve is to the upper left corner, the lower the probability of failed requests is.
%random rounding/sparse area first/dense area first
% \begin{figure}[!htb]
%     \centering
%     \subfigure[.] {
%         \includegraphics[width=0.7\columnwidth]{images/overload_round_error_rate_cdf.pdf}
%     }
%     % \subfigure[xxx.] {
%     %     \label{fig:round_compare:b}
%     %     \includegraphics[width=0.48\columnwidth]{images/.pdf}
%     % }
% \caption{}
% \label{fig:round_compare_cdf}
% \end{figure}


\subsubsection{Average workload vector vs. component-wise max workload vector}
\label{sec:average-max-comparison}
In Section \ref{sec:robust_optimization}, we use the average workload vector as the representative workload vectors. Another option is to use the component-wise max workload vector. There may not be a conclusive answer that one is better than another. We compare these two options using different synthetic traces. As shown in Fig.~\ref{fig:overload_robust_balance_pool}, using average workload vector yields lower workload rejection rate for one trace, but leads to higher rejection rate for the other one.

%using average workload vectors yields much lower workload rejection rate.

%our formulation, we use average historical workload instead of other formats of historical workload.We wish to evaluate the effects of different formats of workload. Apart from the average workload we use, it is natural to make use of the maximum flow of each base station to get the server placement results.

%Similarly, considering the minor difference when testing these methods with real trace, we still use synthetic trace and CDF figure to compare the effects of different methods.


% \begin{figure}[!htb]
%     \centering
%     \subfigure[.] {
%         % \includegraphics[width=0.7\columnwidth]{images/max_mean_compare_cdf.pdf}
%         \includegraphics[width=0.7\columnwidth]{images/overload_robust_balance_pool.pdf}
%     }
%     % \subfigure[xxx.] {
%     %     \label{fig:max_mean_compare:b}
%     %     \includegraphics[width=0.48\columnwidth]{images/.pdf}
%     % }
% \caption{}
% \label{fig:overload_robust_balance_pool}
% \end{figure}

%We consider four conditions in our formulation ,they are respectively the average workload and maximum workload with or without resource pooling idea.Obviously, the CDF curves with average work show better performance. What's more, the function of resource pooling has also been proved with average workloads. On the contrary, based on the maximum workload, we can easily observe its poor performance even if using the resource pooling idea. 

\subsubsection{Understanding the effect of robust optimization and resource pooling} Our server placement policy utilizes both robust optimization and resource pooling to improve its robustness against workload uncertainty. To understand the contribution of each technique, we evaluate four options below:
\begin{enumerate}
    \item \textbf{Robust optimization$+$resource pooling (RO-RP):} Our server placement strategy proposed in Section \ref{sec:server_placement}.
    \item \textbf{Robust optimization only (RO-only):} Only solve (\ref{formulation:server_placement}) for a server placement solution.
    \item \textbf{Resource pooling only (RP-only):} Use only one workload vector (e.g., historical average) to solve (\ref{formulation:server_placement}) \& (\ref{formulation:server_placement_robustification}).
    \item \textbf{Not handling workload uncertainty (TwithLB):} Use only one representative workload vector to solve (\ref{formulation:server_placement}).
\end{enumerate}
From Fig.~\ref{fig:overload_error_rate_cdf_80000}, we can see that both techniques help reduce the workload rejection rate, and the performance is the best when both techniques are enabled.

%compare three conditions including Robustness optimization, Resource Pooling and No Optimization.Unexpectedly, Robustness Optimization has the worst performance and Resource Pooling, without question, performs best.

%Besides proving the functions of rounding schemes and the formats of historical workload, Resource Pooling is the key idea when improving the robustness of our formulation. Therefore, we expect to compare the Resource Pooling with the Robustness Optimization which is also commonly used.And we still evaluate these ideas with synthetic trace in the format of CDF figure.

% \begin{figure}[!htb]
%     \centering
%     \subfigure[.] {
%         % \label{fig:robust_compare:a}
%         % \includegraphics[width=0.7\columnwidth]{images/robust_compare_cdf.pdf}
%         \includegraphics[width=0.7\columnwidth]{images/overload_error_rate_cdf_80000.pdf}
%     }
%     % \subfigure[xxx.] {
%     %     \label{fig:robust_compare:b}
%     %     \includegraphics[width=0.48\columnwidth]{images/.pdf}
%     % }
% \caption{}
% \label{fig:robust_compare_cdf}
% \end{figure}

\subsection{Evaluate Server Scheduling}
The objective of server scheduling is to reduce cost without affecting service quality. We compare three strategies below:
\begin{enumerate}
    \item \textbf{No server scheduling (No-SS):} This strategy turns on all the deployed edge servers at all times.
    \item \textbf{Server scheduling without accounting for the switching cost (SSwithoutSC):} Switching cost can be high. Frequently toggling a server between on/off states may reduce this server's life time.
    \item \textbf{Server scheduling that explicitly accounts for the switching cost (SSwithSC):} This is our final server scheduling strategy. Two settings for the switching cost are evaluated: 1) the switching cost is equal to running a server in idle state for 12 minutes; 2) the switching cost is equal to running a server in idle state for one hour. We also evaluate the number of on-off switchings to demonstrate the benefits of this server scheduling policy.
    %considering the on-off switchings may lead to the loss of servers and reduce the service life of servers.
\end{enumerate}

\begin{figure}[!htb]
    \centering
    % \includegraphics[width=0.8\linewidth]{images/draw_scheduling_final_error.pdf}
    \includegraphics[width=0.8\linewidth]{images/draw_server_scheduling_final_error.pdf}
    \caption{Workload rejection rate under different server scheduling policies.}
    \label{fig:draw_server_scheduling_final_error}
\end{figure}

We first compare the energy consumption of the three strategies in Fig.~\ref{fig:draw_energy_consumption_1}\&\ref{fig:draw_energy_consumption_02}. As expected, with server scheduling, many servers are switched off during idle hours, thus reducing the energy consumption dramatically. In total, server scheduling could save about 13\% of energy consumption. 

However, toggling servers between on/off states may incur additional cost, and thus it is better to minimize the total number of on/off switchings. As shown in Fig.~\ref{fig:draw_energy_consumption_count}, explicitly accounting for the switching cost reduces the total number of switchings by about 80\% compared to SSwithoutSC. 

Finally, we plot Fig.~\ref{fig:draw_server_scheduling_final_error} to evaluate the workload rejection rate before and after performing server scheduling. The takeaway message is that, performing server scheduling could significantly reduce energy cost, without dramatically increasing the workload rejection rate.

%Note that, the cost savings of server scheduling



%Considering the target of server scheduling, our evaluations to the server scheduling schemes are related to two aspects including the energy consumption and the service quality.

%First, according to Fig.~\ref{fig:draw_energy_consumption}, baseline energy consumption represent the energy cost in the condition where all servers stay  active and serve for an hour.The energy consumption curve means the consumption after taking advantage of our server scheduling schemes.
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/draw_energy_consumption.pdf}
%     \caption{xxx.}
%     \label{fig:draw_energy_consumption}
% \end{figure}



% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/draw_energy_consumption_count.pdf}
%     \caption{xxx.}
%     \label{fig:draw_energy_consumption_count}
% \end{figure}


% Clearly, our server scheduling schemes guide the servers to the standby state at the idle time and avoid the waste of the energy.Even though the process to activate servers may use more energy, our server scheduling schemes save lots of energy during the operation time in the long run.

% In Fig.~\ref{fig:draw_energy_consumption}, we have proved that our server scheduling schemes can save much energy.However, we expect to save the cost under the circumstances with high service quality, in other words, small number of failed events. 


% Fig.~\ref{fig:draw_server_scheduling_final_error} tells us the number of failed events in the 360 hours of future. We can acquire even though we have turned off some servers in the idle time, the users can still obtain the service which is seldom rejected.
% %\subsection{How many adjacent base stations are selected?}



==> IWQoS2021(Extended)/sections/9Conclusion.tex <==
\section{Conclusion}
In this paper, we propose a new methodology to design server placement and server scheduling policies that are robust to workload uncertainty. This methodology utilizes robust optimization to provide guarantee for workloads that are within a predetermined uncertainty set, and performs resource pool optimization to improve service quality for out-of-bound workloads. Simulation results demonstrate the effectiveness of this methodology. From a service provider's aspect, the resulting server placement policy reduces the number of required edge servers by about 25\% compared with the state-of-the-art approach and the resulting server scheduling policy reduces the energy consumption by about 13\%.

%We study how to design edge server placement and server scheduling policies under workload uncertainty for 5G networks. We introduce a new metric called \emph{resource pooling factor} to handle unexpected workload bursts. Maximizing this metric offers a strong enhancement on top of robust optimization against workload uncertainty. Using both real traces and synthetic traces, we show that the proposed server placement and server scheduling policies not only demonstrate better robustness against workload uncertainty than existing approaches, but also significantly reduce the cost of service providers. Specifically, the proposed server placement policy reduces the number of required edge servers by about 25\% in order to achieve close-to-zero workload rejection rate; the proposed server scheduling policy reduces the energy consumption of edge servers by about 13\% without causing much impact on the service quality.

==> sections/6Implementation.tex <==
\section{Deployment Details}
This section may not be necessary, just like the other MEC papers.

\subsection{Hardware Interconnection}

\subsection{Software Control}
Describe the software architecture and control ideas needed.

With the help of Cloudlet?

\section{A Close-to-Optimal Algorithm for Server Placement with Polynomial Complexity}
We compute a server placement solution in two steps: 1) ignore the integer requirement on $[S_m]$, and compute a fractional solution first; 2) round the fractional solution of $[s_m]$ to an integer solution using min cost flow.

\subsection{Compute a Fractional Solution}
After removing the integer requirement on $[S_m]$, it is easy to check that (\ref{formulation:server_placement_robustification}) becomes a linear problem problem, which can be solved in polynomial time. However, (\ref{formulation:server_placement}) becomes a bi-linear problem (the constraints (\ref{eqn:server_capacity}) contain a multiplication term between the variables $S_{m}$ and $\beta$), which is still hard to solve. 

Fortunately, (\ref{formulation:server_placement}) can be easily transformed to an linear problem using the following variable substitution:
\begin{equation}\label{eqn:variable_substitution}
u_{mn}^{'} = \frac{u_{mn}w_m}{C\beta}, \kappa = \frac{1}{C\beta}.
\end{equation}
Using $u_{mn}^{'}$ and $\kappa$, the constraints (\ref{eqn:demand_split}) and (\ref{eqn:server_capacity}) are transformed into
\begin{equation}\label{eqn:demand_split_new}
u_{m1}^{'}+u_{m2}^{'}+\cdots+u_{mM}^{'}=w_m\kappa, m=1,2,...,M,
\end{equation}
\begin{equation}\label{eqn:server_capacity_new}
u_{1n}^{'}+u_{2n}^{'}+\cdots+u_{Mn}^{'} \leq S_{n}, n=1,2,...,M.
\end{equation}
The original optimization problem (\ref{formulation:server_placement}) is now transformed into:
\begin{equation}\label{formulation:server_placement_new}
\boxed{
\begin{aligned}
\max_{S_m,u_{mn}^{'},\kappa} & \hspace{20mm}\kappa &\\
\text{s.t.}& \hspace{3mm} S_m,u_{mn}^{'},\kappa\text{ satisfy (\ref{eqn:demand_split_new})(\ref{eqn:total_servers})(\ref{eqn:server_capacity_new})}&\\
&\hspace{3mm}0\leq u_{mn}^{'}\leq w_m\kappa\text{ and } u_{mn}^{'}=0\text{ for }n\notin \Omega_{m}(\delta) &
\end{aligned}
}
\end{equation}
Clearly, if we ignore the integer requirement on $[S_m]$, (\ref{formulation:server_placement_new}) becomes a linear programming problem.

% \begin{equation}
% 	\left\{ 
% 	\begin{array}{c}
% 	u_{11}^{'}(t)+u_{12}^{'}(t)+u_{13}^{'}(t)+\cdots+u_{1M}^{'}(t) = 1/\beta \\ 
% 	u_{21}^{'}(t)+u_{22}(t)+u_{23}^{'}(t)+\cdots+u_{2M}^{'}(t) = 1/\beta  \\ 
% 	\cdots\cdots\cdots\cdots  \\
% 	u_{M1}^{'}(t)+u_{M2}(t)+u_{M3}^{'}(t)+\cdots+u_{MM}^{'}(t) = 1/\beta  \\ 
% 	\end{array}
% 	\right. 
% \end{equation}
% \begin{equation}
% \left\{ 
% \begin{array}{c}
% u_{11}^{'}(t)w_1(t)+u_{21}^{'}(t)w_2(t)+\cdots+u_{M1}^{'}(t)w_M(t) \leq S_{1}*C \\ 
% u_{12}^{'}(t)w_1(t)+u_{22}^{'}(t)w_2(t)+\cdots+u_{M2}^{'}(t)w_M(t) \leq S_{2}*C  \\ 
% \cdots\cdots\cdots\cdots  \\
% u_{1M}^{'}(t)w_1(t)+u_{2M}^{'}(t)w_2(t)+\cdots+u_{MM}^{'}(t)w_M(t) \leq S_{M}*C  \\ 
% \end{array}
% \right. 
% \end{equation}

\subsection{Round the Fractional Solution to An Integer Solution}
Let $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}, \tilde{\eta}$ be the fractional server placement solution obtained from solving (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}) as linear programming problems. Since we have relaxed the integer requirement of $S_m$, the resulting $\tilde{\beta}$ must be a lower bound of the optimal value of (\ref{formulation:server_placement}), while $\tilde{\eta}$ must be an upper bound of the optimal value of (\ref{formulation:server_placement_robustification}). In order to convert the fractional solution to an integer solution, we first introduce some mathematical preliminaries on the min cost circulation problem.

\subsubsection{Mathematical Preliminaries on the Min Cost Circulation Problem}
\begin{definition}\label{mincostcirculation}
(Min-Cost Circulation Problem) Given a flow network with
\begin{itemize}
  \item $l(v,w)$, lower bound on flow from node $v$ to node $w$;
  \item $u(v,w)$, upper bound on flow from node $v$ to node $w$;
  \item $c(v,w)$, cost of a unit of flow on $(v,w)$,
\end{itemize}
the goal of the min-cost circulation problem is to find a flow assignment $f(v,w)$ that minimizes
$$\sum_{(v,w)}c(v,w)\cdot f(v,w),$$
while satisfying the following two constraints:
\begin{enumerate}
  \item Throughput constraints: $l(v,w)\leq f(v,w)\leq u(v,w)$;
  \item Flow conservation constraints: $\sum_u f(u,v) = \sum_w f(v,w)$ for any node $v$.
\end{enumerate}
\end{definition}

Note that all the constant parameters $l(v,w),u(v,w)$ are all positive and $c(v,w)$ can be either positive or negative. In addition, min-cost circulation problem has a very nice property that guarantees integer solutions:
\begin{lemma}\label{integralflowtheorem}
(Integral Flow Theorem) Given a feasible circulation problem, if $l(v,w)$'s and $u(v,w)$'s are all integers, then there exists a feasible flow assignment such that all flows are integers.
\end{lemma}

In fact, for feasible circulation problems with integer bounds, most max-flow algorithms, e.g., Edmonds-Karp algorithm \cite{Edmonds1972Theoretical} and Goldberg-Tarjan algorithm \cite{Goldberg1988A}, are guaranteed to generate integer solutions.

\subsubsection{Mapping the Server Placement Problem to a Min Cost Circulation Problem}

We would like to find an integer solution for $S_m$ satisfying (\ref{eqn:demand_split})(\ref{eqn:total_servers})(\ref{eqn:server_capacity}) around the fractional solution $\tilde{S}_m$. The basic idea is to map these constraints to the flow conservation constraints in the min cost circulation problem. 

\noindent\textbf{Step 1:} Let $\tilde{u}_{mn}^{'} = \frac{\tilde{u}_{mn}w_m}{C\tilde{\beta}}$ and $\tilde{\kappa}=\frac{1}{C\tilde{\beta}}$. We first prove that $\tilde{u}_{mn}^{'}$ and $\tilde{S}_m$ satisfy
\begin{subequations}
\begin{align}
    &\tilde{u}_{m1}^{'}+\tilde{u}_{m2}^{'}+\cdots+\tilde{u}_{mM}^{'}=w_m\tilde{\kappa}, \hspace{3mm}m=1,2,...,M;\label{subeqn:demand_split}\\
    &\tilde{u}_{1n}^{'}+\tilde{u}_{2n}^{'}+\cdots+\tilde{u}_{Mn}^{'}=\tilde{S}_n, \hspace{3mm}n=1,2,...,M;\label{subeq:capacity}\\
    &\tilde{S}_1+\tilde{S}_2+\cdots+\tilde{S}_M=K.\label{subeq:num_servers}
\end{align}
\end{subequations}
(\ref{subeqn:demand_split}) and (\ref{subeq:num_servers}) follow directly from the constraints (\ref{eqn:demand_split}) and (\ref{eqn:total_servers}). However, for (\ref{subeq:capacity}), the constraint (\ref{eqn:server_capacity}) only implies
$$\tilde{u}_{1n}^{'}+\tilde{u}_{2n}^{'}+\cdots+\tilde{u}_{Mn}^{'}\leq \tilde{S}_n.$$
To see why equality holds in (\ref{subeq:capacity}), we use the fact that $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}$ is actually an optimal fractional solution of (\ref{formulation:server_placement}). If the equality in (\ref{subeq:capacity}) does not always hold, we can reduce $\tilde{S}_m$ to $\tilde{S}_m^{'}$ to make the equality in (\ref{subeq:capacity}) hold. In this case, we must have $$\tilde{S}_1^{'}+\tilde{S}_2^{'}+\cdots+\tilde{S}_M^{'}<K.$$
Let $\rho = \frac{\sum_{n=1}^M \tilde{S}_n^{'}}{K}<1$, then it is easy to check that $\frac{1}{\rho}\tilde{S}_m^{'}, \tilde{u}_{mn}, \rho\tilde{\beta}$ is also a feasible fractional solution of (\ref{formulation:server_placement}). However, $\rho\tilde{\beta}<\tilde{\beta}$, which contradicts to the fact that $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}$ is an optimal solution of (\ref{formulation:server_placement}).


\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.44]{./images/min_cost_flow.pdf}
    \caption{The flow graph corresponding to (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}).}
    \label{fig:min_cost_flow}
\end{figure}

\noindent\textbf{Step 2:}
Based on the constraints (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}), we construct a flow graph as follows (also see Fig. \ref{fig:min_cost_flow}):
\begin{enumerate}
  \item Create a directed $M\times M$ bipartite graph. We create $M$ nodes on the left hand side of the bipartite graph, and create $M$ nodes on the right hand side of the bipartite graph. We add a directed link from $m$ to $n$, and set the bounds of this link as $[\lfloor \tilde{u}_{mn}^{'}\rfloor, \lceil\tilde{u}_{mn}^{'}\rceil]$ and the cost of this link as $0$.
  \item Add a source node, $M$ directed links for this source node to the $M$ left nodes. The bounds of the $m$-th link is set as $[\lfloor w_m\tilde{\kappa} \rfloor, \lceil w_m\tilde{\kappa}\rceil]$, and the cost is set to 0. %$\frac{\lfloor w_m\tilde{\kappa} \rfloor}{w_m\tilde{\kappa}}$.
  \item Add a sink node and $M$ directed links from the $M$ right nodes to this sink node. The bounds of the $m$-th link is set as $[\lfloor \tilde{S}_m \rfloor, \lceil \tilde{S}_m\rceil]$, and the cost is set to $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$.
  \item Add a feedback link from the sink node to the source node. The bounds of this feedback link is set as $[K,K]$, and the cost is set to $0$.
\end{enumerate}
In this flow graph, the flow conservation constraint on each left node corresponds to one of the constraints in (\ref{subeqn:demand_split}); the flow conservation constraint on each right node corresponds to one of the constraints in (\ref{subeq:capacity}); and the flow conservation constraint on the sink node corresponds to the constraint (\ref{subeq:num_servers}). Hence, according to (\ref{subeqn:demand_split})-(\ref{subeq:num_servers}), it is easy to construct a feasible flow assignment for the above flow graph as follows:
\begin{enumerate}
    \item Assign $w_m\tilde{\kappa}$ amount of flow to the link between the source node and the $m$-th left node;
    \item Assign $\tilde{u}_{mn}^{'}$ amount of flow to the link between the $m$-th left node and the $n$-th right node;
    \item Assign $\tilde{S}_m$ amount of flow to the link between the $n$-th right node and the sink node;
    \item Assign $K$ amount of flow to the link between the sink node and the source node.
\end{enumerate}

Since all the bounds in the above flow graph are integers, according to Lemma \ref{integralflowtheorem}, this flow graph must have an integer solution with the minimum cost, which can be computed in polynomial time using algorithms like, Edmonds-Karp algorithm~\cite{Edmonds1972Theoretical} and Goldberg-Tarjan algorithm~\cite{Goldberg1988A}. In our own implementation, we have used Google OR-Tools~\cite{OrTools} as our min cost circulation problem solver. After obtaining an integer flow assignment for the above min cost circulation problem, the flow values of the $M$ links between the right nodes and the sink node give the server placement results, which we denote by $[S_1^*,S_2^*,...,S_M^*].$

\noindent\textbf{Remark on the unit cost:} Note that we set the unit cost of the link between the $m$-th right node and the sink node as $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$. The reason is that we want to minimize the rounding loss. $\frac{\lfloor \tilde{S}_m \rfloor}{\tilde{S}_m}$ can be interpreted as the remaining fraction of capacity after rounding down. If this number is small, we should try to avoid rounding down. This step is critical for our min cost circulation based approach to achieve close to optimal performance.

\noindent\textbf{Remark on the optimality:} Rigorously speaking, the min cost flow based approach is not optimal. However, as the edge workload increases, more servers will be deployed. As a result, the values of $\tilde{S}_m$ become large, and  $S_m^*/\tilde{S}_m$ approaches to 1 because $S_m^*\in [\lfloor \tilde{S}_{m}\rfloor, \lceil\tilde{S}_{m}\rceil]$. As $S_m^*/\tilde{S}_m$ approaches to 1, the objective values of (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}) also approach the performance bound $\tilde{\beta}$ and $\tilde{\eta}$.

\noindent\textbf{Versus native rounding approaches:} Our min cost circulation based rounding approach seems complicated. Readers may question the necessity of using such a approach. In fact, before proposing this min cost circulation based rounding approach, we have tried some naive rounding approaches. However, these rounding approaches exhibit poor performance (see \S\ref{}).

% \noindent\textbf{Step 3: Understanding the Performance Gap.} The essence of the min cost flow based approach is to imitate the fractional solution as much as possible. That is why we expect it to have close-to-optimal performance in practice. Next, we provide some theoretical analysis on its performance. We also conduct numerical analysis in \S\ref{}.

% Let $S_m^*, u_{mn}^*, \beta^*, \eta^*$ be the optimal server placement solution obtained by solving (\ref{formulation:server_placement}) and (\ref{formulation:server_placement_robustification}).
% Let $\tilde{S}_m, \tilde{u}_{mn}, \tilde{\beta}, \tilde{\eta}$ be the optimal fractional server placement solution, and let $S_m^{**}, u_{mn}^{**}, \beta^{**}, \eta^{**}$ be the server placement solution obtained using the min cost circulation based approach. 


%For the server placement model and server scheduling model ,considering the number of servers $S_{n}$  and the number of operating servers $S_{n}(t)$ in AP $A_{n}$ are all integers, we use integer programming to solve the problem. But integer programming has high complexity which may consume lots of time to get the solution. As a consequence, considering the linear programming's low complexity, we decide to transfer 

% We prove the following theorem:
% \begin{theorem}\label{thm:circulation}
% Consider the following ILP:
% \begin{eqnarray}\label{eqn:general_form}
% &\min\limits_{\mathbf{a}=[a_{ij}]}& \sum_{i=1}^I\sum_{j=1}^J C_{ij}a_{ij}\\
% &\text{s.t.}&A_{ij}^L \leq a_{ij} \leq A_{ij}^U, \quad \forall \; i,j=1,...,N,\nonumber\\
% &&P_j^L\leq \sum_{i=1}^I a_{ij}\leq P_j^U,\quad \forall \; j=1,...,N,\nonumber\\
% &&Q_i^L\leq \sum_{j=1}^J a_{ij}\leq Q_i^U,\quad \forall \; i=1,...,N,\nonumber
% \end{eqnarray}
% where ${\bf a}=[a_{ij}]$ is an $I\times J$ matrix, and ${\bf C}=[C_{ij}], {\bf P}^L=[P_j^L], {\bf Q}^L=[Q_i^L], {\bf P}^U=[P_j^U], {\bf Q}^U=[Q_i^U], {\bf A}^L=[A_{ij}^L], {\bf A}^U=[A_{ij}^U]$ are integer constants. (Note that ${\bf C}=[C_{ij}]$ can be negative.) If (\ref{eqn:general_form}) has a fractional solution, then (\ref{eqn:general_form}) must have an integer solution, which can be solved in polynomial time.
% \end{theorem}
